Group Property Inference Attacks Against Graph Neural Networks

With the fast adoption of machine learning (ML) techniques, sharing of ML models is becoming popular. However, ML models are vulnerable to privacy attacks that leak information about the training data. In this work, we focus on a particular type of privacy attacks named property inference attack (PIA) which infers the sensitive properties of the training data through the access to the target ML model. In particular, we consider Graph Neural Networks (GNNs) as the target model, and distribution of particular groups of nodes and links in the training graph as the target property. While the existing work has investigated PIAs that target at graph-level properties, no prior works have studied the inference of node and link properties at group level yet. In this work, we perform the first systematic study of group property inference attacks (GPIA) against GNNs. First, we consider a taxonomy of threat models under both black-box and white-box settings with various types of adversary knowledge, and design six different attacks for these settings. We evaluate the effectiveness of these attacks through extensive experiments on three representative GNN models and three real-world graphs. Our results demonstrate the effectiveness of these attacks whose accuracy outperforms the baseline approaches. Second, we analyze the underlying factors that contribute to GPIA's success, and show that the target model trained on the graphs with or without the target property represents some dissimilarity in model parameters and/or model outputs, which enables the adversary to infer the existence of the property. Further, we design a set of defense mechanisms against the GPIA attacks, and demonstrate that these mechanisms can reduce attack accuracy effectively with small loss on GNN model accuracy.

==> text/agg-comp.tex <==
\begin{figure}[t!]
    \centering
%   \vspace{0.1in}
      \centering
      \includegraphics[width=0.45\textwidth]{text/figure/agg-embed-legend(2)(1).pdf}\\
   \includegraphics[width=0.45\textwidth]{text/figure/gcn-agg-comp.pdf}
     \vspace{-0.1in}
    % \caption{GCN}
\caption{\label{fig:dif-ft-embedding-aggregation} Impacts of embedding aggregation methods - concatenation ($F_1$), mean-pooling ($F_2$), max-pooling ($F_3$) - on GPIA performance. }
%$Z^1$, $Z^2$, and $Z^{1,2}$ are indicated in different colors respectively, while $F_1$(concatenation), $F_2$ (mean-pooling), and $F_3$ (max-pooling) are indicated in solid, horizontal stripe, and diagonal stripe fill respectively.}
 \vspace{-0.1in}
\end{figure}
\nop{
\begin{figure*}[t!]
    \centering
%   \vspace{0.1in}
      \centering
      \includegraphics[width=0.7\textwidth]{text/figure/agg-comp-legend(2).pdf}\\
   \includegraphics[width=0.7\textwidth]{text/figure/gcn-embed-agg.pdf}
     \vspace{-0.1in}
    % \caption{GCN}
\caption{\label{fig:dif-ft-embedding-aggregation} Impacts of embedding aggregation methods on PIA performance. $F_1$: Concatenation, $F_2$: Mean-pooling, $F_3$: Max-pooling. \Wendy{change the colors to be the following: same embeddings use the same color (e.g., blue for z1), and the same embedding aggregation method with the same filling (e.g., F1 use shade, F2 use vertical line, F3 use horizontal line, etc.)}} 
\end{figure*}
}

==> text/analysis.tex <==
\section{Factors that Impact PIA Performance}

%\input{text/correlation}

\nop{
\begin{table*}[t!]
    \centering
    \begin{tabular}{|c|c|c|c|c|}\hline
        Task &Graph & \# of Node features for training& Classification task / \# of Classes& Properties to be attacked  / \# of Classes\\\hline
         T6 &Pokec & 4 (A,H,W,R) &public / 2 &portion of male / 2\\\hline
         T7 &Pokec & 4 (G,H,W,R) &public / 2 &portion of (age > 20) / 2\\\hline
        T8 &Pokec & 4 (P,A,H,R) &gender / 2 &portion of (weight > 60KG) / 2\\\hline
        T9 &Pokec & 3 (P,A,R) &gender / 2 &portion of (weight > 60KG) / 2\\\hline
        T10 &Pokec & 2 (P,R ) &gender / 2 &portion of (weight > 60KG) / 2\\\hline
         T11 &Pokec & 2 (2 random values of P,R ) &gender / 2 &portion of (weight > 60KG) / 2\\\hline
        T12 &Pokec & 5 (P,A,H,W,R) &public / 2 &portion of (age > 20) / 4\\\hline
        T13 &Pokec & 5 (P,A,H,W,R) &public / 2 &portion of (age > 20) / 8\\\hline
    \end{tabular}
    \caption{Datasets and their properties to be attacked ( P-public, G-gender, A-age, H-heights, W-weight, R-region) \Wendy{why not use A1 - A7?} \xiuling{I put A6,A7 in section 5.1 to see the impact of "Whether the target model sees the target feature of PIA task in training", and if we put A6 A7 here, figure 1 will be very crowed. }}
    \label{tab:data2}
\end{table*}
}

\subsection{Data Properties}

\Wendy{Also can measure node and link  importance measured by saliency maps.  Code and tutorial are available at: https://stellargraph.readthedocs.io/en/stable/demos/interpretability/gcn-node-link-importance.html}
\noindent{\bf Importance of property feature.} 
We measure the {\em importance of the property feature} as the difference in the target model performance on the training data with and without the property feature $P$. The sesults are shown in Table \ref{tab:compare1}.

\xiuling{\noindent{\bf Impact of node features which are highly related to property feature.}} We remove the node features that are highly related to property feature as the difference in the target model training data.


% \begin{figure*}[t!]
%     \centering
% %   \vspace{0.1in}
% \begin{tabular}{ccc}
%     \begin{subfigure}[b]{.3\textwidth}
%       \centering
%     %  \includegraphics[width=\textwidth]{text/figure/gcn-pia.pdf}
%     \includegraphics[width=\textwidth]{text/figure/gcn-a1-acc-pclasses.pdf}
%      \vspace{-0.2in}
%     \caption{GCN}
%     \end{subfigure}
%     &
%     \begin{subfigure}[b]{.3\textwidth}
%     \centering
%     % \includegraphics[width=\textwidth]{text/figure/graphsage-pia.pdf}
%     \includegraphics[width=\textwidth]{text/figure/graphsage-a1-acc-pclasses.pdf}
%     \vspace{-0.2in}
%     \caption{GraphSage}
%     \end{subfigure}
%     &
%     \begin{subfigure}[b]{.3\textwidth} 
%     \centering
%     \includegraphics[width=\textwidth]{text/figure/gat-a1-acc-pclasses.pdf}
%     \vspace{-0.2in}
%     \caption{GAT}
%     \end{subfigure}
% \end{tabular}    
%     \vspace{-0.05in}
% \caption{\label{fig:pia_acc_pclasses} Attack accuracy for different number of property classes.} 
% \end{figure*}

\subsection{Model Properties}







==> text/attack-model.tex <==
\section{Methodology}
 \label{sc:method}

\begin{table}
    \centering
    \begin{tabular}{c|c|c|c}
    \hline
         \multirow{2}{*}{\textbf{Attack}}& \multicolumn{3}{c}{\textbf{Adversary knowledge}} \\\cline{2-4}
          & {$\ShadowG$} & Access to {$\TargetM$} & {$\PartialG$}\\\hline
          $A_1$ & $\times$ & White-box & $\checkmark$ \\\hline
          $A_2$ & $\times$ & Black-box & $\checkmark$ \\\hline
         $A_3$ & $\checkmark$ & White-box & $\times$ \\\hline
         $A_4$ & $\checkmark$ & Black-box & $\times$ \\\hline
          $A_5$ & $\checkmark$ & White-box & $\checkmark$ \\\hline
         $A_6$ & $\checkmark$ & Black-box & $\checkmark$ \\\hline
    \end{tabular}
    \caption{Attack taxonomy ($\ShadowG$: shadow graph; $\TargetM$: target model; $\PartialG$: partial graph).}
    \label{tab:attacks}
    \vspace{-0.2in}
\end{table}

\nop{
\begin{table}
    \centering
    \begin{tabular}{c|c|c|c|c}
    \hline
         \multirow{2}{*}{\textbf{Attack}}& \multicolumn{3}{c|}{\textbf{Adversary knowledge}} & \multirow{2}{*}{\bf Feature dimension size}  \\\cline{2-4}
          & {$\ShadowG$} & {$\TargetM$} & {$\PartialG$}\\\hline
          $A_1$ & $\times$ & White-box & $\checkmark$ & {$s \cdot agg(\mathbb{R}^{n \times d})$} \\\hline
          $A_2$ & $\times$ & Black-box & $\checkmark$ & {$s \cdot agg(\mathbb{M}^{n \times l})$}\\\hline
         $A_3$ & $\checkmark$ & White-box & $\times$ & $s \cdot Align( agg(\mathbb{R}^{n \times d}))$\\\hline
         $A_4$ & $\checkmark$ & Black-box & $\times$ & $s \cdot Align( agg(\mathbb{M}^{n \times l}))$\\\hline
          $A_5$ & $\checkmark$ & White-box & $\checkmark$ & { $s \cdot agg(\mathbb{R}^{n \times d})$} \\\hline
         $A_6$ & $\checkmark$ & Black-box & $\checkmark$ & {$ s \cdot agg(\mathbb{M}^{n \times l})$}\\\hline
    \end{tabular}
    \caption{Attack taxonomy. $\ShadowG$: shadow graph; $\TargetM$: target model; $\PartialG$: partial graph. \xiuling{$s$ is the number of GPIA training graphs, $agg()$ is the aggregation method, $\mathbb{R}^{n \times d}$ is the embedding matrix with dimension of $n \times d$ for each graph in $s$, $n$ is number of nodes in each graph, $d$ is the embedding dimension, $\mathbb{M}^{n \times l}$ is the posterior metric with dimension of $n \times l$ for each graph in $s$, $n$ is number of nodes in each graph, $l$ is the number of classification labels. For white-box attacks, if $agg()$ is max-pooling or mean-pooling, $\mathbb{R}^{n \times d}=\mathbb{R}^{n \times 1}$, if $agg()$ is concatenation $\mathbb{R}^{n \times d}=\mathbb{R}^{1 \times (n*d)}$. For black-box attacks, if $agg()$ is concatenation $\mathbb{M}^{n \times l}=\mathbb{M}^{1 \times (n*l)}$, if $agg()$ is element-wise differences, $\mathbb{M}^{n \times l}=\mathbb{M}^{n \times 1}$. $Align()$ is the dimension alignment method, if $Agg()$ is $Sampling$, $Align(agg(\mathbb{R}^{n \times d}))= agg(\mathbb{R}^{n \times d})$, if $Agg()$ is $TSNE$, $Align( agg(\mathbb{R}^{n \times d}))= d_{TSNE}$, $d_{TSNE}$ is the dimension after TSNE projection, which is 2 or 3, if $Agg()$ is $PCA$, $Align(agg(\mathbb{R}^{n \times d}))= d_{PCA}$, $d_{PCA}$ is the dimension to be preserved, if $Agg()$ is $Autoencoder$, $ Align( agg(\mathbb{R}^{n \times d}))= d_{Enc}$, $d_{Enc}$ is the dimension of encoder} \Wendy{You can revise the table structure.}}
    \caption{Attack taxonomy. $\ShadowG$: shadow graph; $\TargetM$: target model; $\PartialG$: partial graph. $s$: \# of shadow graphs}
    \label{tab:attacks}
    \vspace{-0.2in}
\end{table}

 
\begin{table}[t!]
    \centering
    \begin{tabular}{c|c|c|c|c|c}
    \hline
         \multirow{3}{*}{\textbf{Attack}}& \multicolumn{3}{c|}{\textbf{Adversary knowledge}} & \multicolumn{2}{c}{\bf Feature dimension size}  \\\cline{2-6}
          & \multirow{2}{*}{$\ShadowG$} & \multirow{2}{*}{$\TargetM$} & \multirow{2}{*}{$\PartialG$} & Before  & After  \\
          & & & & alignment & alignment \\\hline
          $A_1$ & $\times$ & White-box & $\checkmark$ & \multicolumn{2}{c}{$s \cdot agg(\mathbb{R}^{n \times d})$} \\\hline
          $A_2$ & $\times$ & Black-box & $\checkmark$ & \multicolumn{2}{c}{$s \cdot agg(\mathbb{M}^{n \times l})$}\\\hline
         $A_3$ & $\checkmark$ & White-box & $\times$ &$s \cdot agg(\mathbb{R}^{n \times d})$ & $s \cdot Align(agg(\mathbb{R}^{n \times d}))$\\\hline
         $A_4$ & $\checkmark$ & Black-box & $\times$ &$s \cdot agg(\mathbb{R}^{n \times d})$ & $s \cdot Align(agg(\mathbb{M}^{n \times l}))$\\\hline
          $A_5$ & $\checkmark$ & White-box & $\checkmark$ & \multicolumn{2}{c}{$s \cdot agg(\mathbb{R}^{n \times d})$} \\\hline
         $A_6$ & $\checkmark$ & Black-box & $\checkmark$ & \multicolumn{2}{c}{$s \cdot agg(\mathbb{M}^{n \times l})$}\\\hline
    \end{tabular}
    \caption{Attack taxonomy. $\ShadowG$: shadow graph; $\TargetM$: target model; $\PartialG$: partial graph. \Wendy{You can revise the table structure.}}
    \label{tab:attacks}
    \vspace{-0.2in}
\end{table}
}

The goal of GPIA is to design a binary classifier $\PIA$ that predicts whether the training graph $\Ttrain$ has a pre-defined property $\Property$.  
Then, the attack's goal can be formulated as: $\PIA: \ExternalK, \Property  \rightarrow L$, 
where $\mathcal{K}$ denotes the adversary knowledge, and $L$ is the set of class labels for property prediction.  In this paper, we only consider binary property (i.e., $L=\{0, 1\}$). We will discuss how to extend to non-binary properties in Section \ref{sc:conclusion}.


Whether the adversary has each of $\PartialG$, $\TargetM$, and $\ShadowG$ in $\ExternalK$ is a binary choice. However, we assume at least one of  $\PartialG$ and $\ShadowG$ is available for training of GPIA model, as the adversary always can obtain some public graphs from external resources as the shadow graphs if the partial graph is not available. Therefore, we have a comprehensive taxonomy with six different threat models based on different combinations of $\PartialG$, $\TargetM$, and $\ShadowG$ in $\ExternalK$. We design six GPIA attack classifiers for these threat models, and summarize the taxonomy of our  attacks in Table \ref{tab:attacks}. Next, we describe the details of the black-box attacks ($A_2, A_4, A_6$) first, followed by the details of the white-box attacks ($A_1, A_3, A_5$).  
% \Wendy{Add a paragraph highlighting the novelty of our shadow model.}
\nop{
\begin{table}[t!]
    \centering
    \begin{tabular}{c|c|c|c}
    \hline
       \multirow{2}{*}{Attack} & \multirow{2}{*}{Attack type} & \multicolumn{2}{c}{\bf Feature dimension size}\\\cline{3-4}
       & & Before alignment & After alignment \\\hline
        $A_1$ & White-box & & \\\hline
        $A_2$ & Black-box & &N/A \\\hline
        $A_3$ & White-box & & \\\hline
        $A_4$ & Black-box & & N/A\\\hline
        $A_5$ & White-box & & \\\hline
        $A_6$ & Black-box & & N/A\\\hline
    \end{tabular}
    \caption{Comparison of six attacks}
    \label{tab:attack-feature}
    \vspace{-0.2in}
\end{table}
}
\nop{
We design two types of attacks in terms of different adversary knowledge $G_{ack}$: 
\begin{itemize}
    \item {\bf Black-box attack} for the adversary who can access the target model output only. As we only consider the node classification task in this paper, we consider the probability posteriors generated by the target GNN model as the input to the black-box attack.   
    \item {\bf White-box attack} when the adversary has access to the target model, including the model's architecture and parameter values. 
\end{itemize}
}


\subsection{Black-box Attacks}
\label{sc:black-box-ttack}
 \begin{figure*}[t!]
\begin{center}
\includegraphics[width=0.95\textwidth]{text/figure/PIA_PLOT.pdf}
%\vspace{-0.1in}
\caption{\label{figure:pia-attack} Overview of the black-box GPIA. \textsf{Agg}() is the aggregation function that generates GPIA features from posteriors.}
\end{center}
\vspace{-0.1in}
\end{figure*}


%We adapt the shadow model approach \cite{shokri2017membership} to enable the adversary to train a set of shadow models that replicate the functionality of the target GNN model. Based on the shadow models, we design a supervised classifier $f$ that is trained on the $G_{ack}$ generated by the shadow models on $G_{aux}$ as well as the labels of ${G_{P}}$. 
The black-box attack includes three phases: {\em shadow model training}, {\em attack model training}, and {\em property attack inference} (Figure \ref{figure:pia-attack}). Next, we explain the details of these three phases. 

{\bf Shadow model training phase.} To collect the data $\Ptrain$ to train the GPIA classifier $\PIA$, first, the adversary trains $k\geq 1$ shadow models ${\ShadowM_{1}}$, $\dots, {\ShadowM_k}$. 
The training data for each shadow model ${\ShadowM_{i}}$ is a subgraph ${\ShadowG_{i}}$ that is randomly sampled from  the partial graph $\PartialG$ (Attack $A_2$), the shadow graph $\ShadowG$ (Attack $A_4)$, or both (Attack $A_6$). 
Each shadow training graph ${\ShadowG_{i}}$ may or may not have the property $\Property$. 
In this paper, we assume all shadow graphs have the same size. Let $n_s$ be the number of nodes in the shadow graphs. Intuitively, to ensure the shadow models mimic the behaviors of the target model, they should be trained in the way that the output of each shadow model  ${\ShadowM_{i}}$ on the shadow training dataset ${\ShadowG_{i}}$ is close to the output of the target model $\TargetM$ on ${\ShadowG_{i}}$. In this paper, we follow the prior works \cite{ateniese2013hacking,ganju2018property} and consider the strongest attack scenario that the shadow models are identical to the target model, i.e.,  they have the same architecture and parameters. 

{\bf Attack model training phase.} 
Before training the GPIA classifier, the adversary constructs the attack training data $\Ptrain$ by the following procedure.  
 For each trained shadow model $\ShadowM_{i}$ and its training data $\ShadowG_i$, the adversary aggregates the set of posterior probability values generated by  $\ShadowM_{i}$ on $\ShadowG_i$ into a vector $\vec{v_i}$.  The vector $\vec{v_i}$ is inserted into the GPIA training dataset $\Ptrain$ as the features, which is associated with a GPIA label “1” if $\ShadowG_i$ is positive, and “0” otherwise. 
 
How to aggregate multiple posterior probability values into one vector as the GPIA features? We consider two different approaches:

\begin{ditemize}
    \item  {\em Concatenation:} Given $n_s$ nodes in the shadow graph, each associated with $\ell$ posterior probabilities, there are $N=n_s\times\ell$ posterior probability $p_1, \dots, p_N$ in total. These $N$ probability values are concatenated 
    into a vector $\vec{v}= <p_1, \dots, p_N>$ as GPIA features.  
    
    \item  {\em Element-wise difference} (EWD): 
For each node $v$, which is associated with $\ell$ posterior probability values $p_1, \dots, p_\ell$, we calculate the {\em average element-wise difference} $p^{\text{diff}}$ of $v$ as follows:
    \[p^{\text{diff}}=\frac{1}{\ell(\ell-1)}\sum_{1\leq i, j\leq \ell, i\neq j}(|p_i - p_j|).\] 
    
    Intuitively, the more (less, resp.) skewed posterior distribution, the higher (lower, resp.) $p^{\text{diff}}$ will be. In a uniform distribution of posteriors, $p^{\text{diff}}=0$.
    After the element-wise difference of each node is calculated, all values are concatenated into a vector $\vec{v}= <p_1^{\text{diff}}, \dots, p_{n_s}^{\text{diff}}>$ as GPIA features. 
     
    \end{ditemize}
    
    The intuition behind the EWD method is that the posterior distributions of positive and negative graphs will be  significantly different, where such difference can be captured by the element-wise difference value. 


 %We will discuss how these two different aggregation methods impact the performance of PIA in Section \ref{sc:exp-pia}.

After $\Ptrain$ is generated, the adversary trains the GPIA classifier $\PIA$ on $\Ptrain$. In this paper, we consider three types of  classifiers, namely Multi-layer Perceptron (MLP), Random Forest (RF), and Linear Regression (LR). 

{\bf Property attack inference phase.} At inference time, the adversary computes the aggregated posterior probability output by the target model $\TargetM$ on the target graph $\TargetG$, using the same posterior aggregation function in the training phase. Then the adversary feeds the aggregated posterior as the input feature of the testing sample to $\PIA$, and obtains the predicted GPIA label. 

\subsection{White-box Attacks}
\label{sc:white-attack}

Unlike the black-box attacks that need shadow models, the white-box attacks do not need any shadow model due to its white-box access to the target model. Therefore, the white-box attacks only include two phases, namely, {\em attack model training} and {\em property attack inference}. Next, we discuss the details of these two phases. 

{\bf Attack model training phase.}  since the adversary has the white-box access to the target model $\TargetM$, he will construct the attack training data $\Ptrain$ by using the model parameters of $\TargetM$ as the features in $\Ptrain$. The motivation behind this is that the parameters of the models trained on the positive graphs will be more similar  than those trained on the negative graphs.
Following this, we design the following method to construct $\Ptrain$. 
For each shadow graph $\ShadowG_{i}$, the adversary uses it to train $\TargetM$ and obtains all the parameters of $\TargetM$, where the parameters are the node embeddings of $\ShadowG_{i}$. The shadow graph $\ShadowG_{i}$ can be randomly sampled from  the partial graph $\PartialG$ (Attack $A_1$), the shadow graph $\ShadowG$ (Attack $A_3)$, or both (Attack $A_5$). Then the adversary  aggregates these node embeddings into a vector $\vec{v_i}$, and inserts $\vec{v_i}$ into $\Ptrain$ as the features. 
He further associates $\vec{v_i}$ with a GPIA label “1” if $\ShadowG_i$ is positive, and “0” otherwise. 

In general, given a GNN model of $k$ layers, the adversary  can choose any $k'\leq k$ layers, and collect the node embeddings of these $k'$ layers to generate GPIA features. We use $A_i^{j_1, \dots, j_t}$ to indicate that the attack $A_i$ uses the model parameters (i.e., node embeddings) at the $j_1$-th, $\dots$, $j_t$-th layers of GNN. For example, $A_1^{2}$ indicates the attack $A_1$ that utilizes the embedding at the 2nd layer of the target model $\TargetM$, and $A_1^{1, 2}$ indicates the attack $A_1$ that utilizes the embeddings at both the 1st and 2nd  layers of $\TargetM$. 
 There are $2^{k}-1$ possible choices of choosing these $k'$ layers in total. 
 Besides these embeddings, the posterior probabilities also can be included to generate features in the same way as in the black-box setting (Section \ref{sc:black-box-ttack}). We will investigate the impact of choosing different amounts of node embeddings on GPIA performance later (Section \ref{sc:exp-pia}). 
 %\Wendy{Xiuling, do you have any experiment result to show that the attack uses the parameters at multiple layers is no better than using the parameters at individual layers  alone? This will reduce the number of possible choices from  $2^{l}-1$ to $l$. Otherwise, you need to justify why you only consider the parameters at one layer but not the parameters of multiple layers.}

Next, we discuss how to aggregate a set of node embeddings into one vector as the GPIA feature. 
%We adapt the pooling methods that are widely used by Convolutional Neural Network (CNN) architecture to “accumulate” features \cite{goodfellow2016deep,boureau2010theoretical}  to our setting.  Specifically, 
We consider the following three aggregation methods in this paper. We adapt two pooling methods that have been widely used for Convolutional Neural Networks  \cite{boureau2011ask,weng1992cresceptron,lecun1998gradient}, namely {\em max-pooling} and {\em mean-pooling}. Both pooling methods take a set of network parameters in the format of vectors as the input, and summarize these vectors as a single vector of fixed length. Max-pooling preserves the most prominent features, while mean-pooling has a smoothing effect.
\begin{ditemize}
   \item {\em Concatenation}: Given $n_s$ node embeddings $z_1, \dots, z_{n_s}$ of the shadow graph, they are concatenated into a vector $\vec{v}=<z_1, \dots, z_{n_s}>$ of dimension $n_s$ as GPIA features.  
    \item {\em Max-pooling}: Given $n_s$ node embeddings $z_1, \dots, z_{n_s}$ from the shadow graph, we generate a vector $\vec{v}=<z^{max}_1, \dots, z^{max}_{n_s}>$ as the GPIA features, where $z^{max}_i$ is the maximum of all value in the embedding $z_i$. 
    \item {\em Mean-pooling}: Given $n_s$ node embeddings $z_1, \dots, z_{n_s}$, we generate a vector $\vec{v}=<z^{mean}_1, \dots, z^{mean}_{n_s}>$, where $z^{mean}_i$ is the mean of all values in $z_i$. 
\end{ditemize}


%Intuitively, given $n_i$ nodes in the shadow graph $\ShadowG_i$, the dimension of $\vec{v_i}$ by the concatenation method is $n_i\times d$, where $d$ is the dimension of node embedding, while the dimension of $\vec{v_i}$ by both max- and mean- pooling methods is $n_i$. Nevertheless, the dimension of $\vec{v_i}$ is determined by the number of nodes in $\ShadowG_i$. 

Different aggregation methods generate different GPIA features, and thus lead to different attack performance. We will investigate the impact of different embedding aggregation methods on GPIA performance in Section \ref{sc:exp-pia}. 

{\bf Property attack inference phase.} At inference time, the adversary collects the model parameters of the target model $\TargetM$ trained on the target graph $\TargetG$, and aggregates the parameters into a vector as the input feature of the testing sample,  by using the same embedding aggregation function in the training phase. Therefore, the feature $\Ptest$ is a vector whose size is the same as the number of nodes in $\TargetG$, whereas the feature of $\Ptrain$ is a vector whose size is the same as the number of nodes in $\ShadowG$. Since $\TargetG$ and $\ShadowG$ may have different number of nodes, the feature of $\TargetG$ and $\ShadowG$ can be of different sizes. This raises the challenge of how to predict on $\Ptest$ if its feature is not of the same size as that of $\Ptrain$.  
\nop{
\begin{table*}
    \centering
    \begin{tabular}{c|c|c|c|c|c}
    \hline
         {\bf Attack type}& {\bf Attack} & {\bf \# of samples} & {\bf Dimension} & {\bf Aggregation function} & {\bf Length of feature (as a vector)}\\\hline
         \multirow{3}{*}{White-box}&\multirow{3}{*}{$A_1, A_3, A_5$}& \multirow{6}{*}{$N_s$}&\multirow{3}{*}{1}&Concatenation & $n_s\times d$\\\cline{5-6}
         & & & &Max-pooling & $n_s$\\\cline{5-6}
         & & & &Mean-pooling & $n_s$\\\cline{1-2}\cline{4-6}
         \multirow{2}{*}{Black-box}&\multirow{2}{*}{$A_2, A_4, A_6$}&
      & \multirow{2}{*}{1}&Concatenation & $n_s\times \ell$ \\\cline{5-6}
         & & & &Element-wise difference & $n_s$\\\hline\hline
         \multicolumn{2}{c|}{Meta-classifier \cite{ateniese2013hacking,ganju2018property}}& $N_s$ & $n_s$ & N/A & $d$ \\\hline
         \end{tabular}
    \caption{\label{tab:attack-dimension} Feature dimension and \# of samples  of training dataset $\Ptrain$ for our six attacks and the meta-classifier method \cite{ateniese2013hacking,ganju2018property} ($N_s$: \# of shadow graphs used to generate GPIA training data; $n_s$: \# of nodes in a shadow graph; $d$: dimension of node embedding, $\ell$: \# of class labels). }
    %\xiuling{does the column of $\bf \# of features$ mean $\bf \# of features per sample$? if so, 1 is not accurate, it should be a vector}\xiuling{My implementation of mea-classifier is in this way, and don't know what you tink about meta-classifier: we averagely partition our GPIA training set to five parts, each parts has the same size of graphs with or w/o property, then we train five classifiers for each part, finally we feed the PIA testing data to each classifier and do majority voting of all the classifiers to get the final decision of whether the testing graphs are with or w/o property. }}  
    \vspace{-0.2in}
\end{table*}
}

To address this challenge, we consider four different to align the features of $\Ptrain$ and $\Ptest$ to be of same dimensions. Next, we explain these four dimension alignment methods in details: (1) \underline{Sampling}: the most straightforward approach is to ensure that $\TargetG$ and $\ShadowG$ have the same number of nodes. This can be achieved as the adversary  can obtain the knowledge of the number of nodes in $\TargetG$ by counting the number of node embeddings via its white-box access to the target model. Then the adversary samples the same number of nodes from $\ShadowG$. This method is applicable when the number of nodes in $\ShadowG$ is no less than that of $\TargetG$; (2) \underline{TSNE projection} \cite{van2008visualizing}: it is a dimension reduction method that projects high-dimensional data to either two or three-dimensional data. We apply TSNE on the features of $\Ptrain$ and $\Ptest$ to project them into the same two-dimensional space, regardless of their original dimensions; (3) \underline{PCA dimension reduction} \cite{minka2000automatic}: it is a widely-used dimension reduction method in the literature. We apply PCA on the feature vector of 
    both $\Ptrain$ and $\Ptest$ and project them into a space of the same dimension; (4) \underline{Autoencoder dimension compression}: Autoencoder \cite{hinton2006reducing} compresses the dimensions in the way that the data in the high-dimensional space can be reconstructed from the representation of lower dimension with small error.  We apply Autoencoder on the features of 
    $\Ptrain$ and $\Ptest$ to compress both into the same space of a lower dimension. 
    To reduce the amounts of information loss by compression, we only compress the feature vector of the larger dimension into the space of the feature vector of smaller one. 

Different alignments methods incur different amounts of information loss on the resulting embeddings, and thus lead to different GPIA performance. We will investigate the impact of different alignment methods on GPIA performance in Section \ref{sc:exp-pia}.

\nop{
{\bf Meta-classifiers \cite{ateniese2013hacking,ganju2018property} versus ours.} The training data $\Ptrain$ of six GPIA classifiers have different feature dimension sizes. We summarize the  number of samples and features of $\Ptrain$  for these attacks in Table \ref{tab:attack-dimension}. If we follow the meta-classifier method \cite{ateniese2013hacking,ganju2018property}, all the parameters of the shadow model can be considered as the features of $\Ptrain$. If we only consider node embeddings as the parameters of GNN models, the feature dimension of $\Ptrain$ for the meta-classifier is the same as the number of nodes in the shadow graph, which can be thousands or  more. 
Training of such meta-classifier is expected to suffer from {\em curse of dimensionality} \cite{}. 
On the contrary, our attacks only have one feature, which contains the information aggregated from all node embeddings in the shadow graph. We will show that the aggregated information  still enables effective PIA (Section \ref{sc:exp-pia}). We note that, although our GPIA features may be of large size, the alignment methods  will reduce the feature length. 
}


==> text/attack34-compare.tex <==
\begin{table*}[t!]
    \centering
    \scalebox{0.9}{\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c}\hline
  \multirow{3}{*}{\bf Target dataset}&\multicolumn{12}{c}{\bf Shadow dataset}\\\cline{2-13}
   &\multicolumn{4}{c|}{Pokec}&\multicolumn{4}{c|}{Facebook}&\multicolumn{4}{c}{Pubmed}\\\cline{2-13}      
   &Sampling&AutoEncoder&PCA&TSNE&Sampling&AutoEncoder&PCA&TSNE&Sampling&AutoEncoder&PCA&TSNE\\\hline
   Pokec&\multicolumn{4}{c|}{N/A}&0.55&0.54&0.53&0.54&0.52&0.50&0.56&0.61\\\hline
   Facebook&0.60&0.51&0.55&0.66&\multicolumn{4}{c|}{N/A}&0.54&0.5&0.56&0.54\\\hline  
   Pubmed&0.58&0.51&0.6&0.71&0.57&0.53&0.58&0.59&\multicolumn{4}{c}{N/A}\\\hline
   \end{tabular}}
   \caption{\label{tab:attack34-compare} Impact of the dimension alignment methods on GPIA performance (GCN as the GNN model, Attack 3 as the attack, $P_1 - P_3$ as the target properties). The three N/A cases do not need dimension alignment as both target and shadow datasets are the same. \Wendy{Merge this table with Table 10, and keep it in appendix.}}
   \end{table*}

==> text/correlation.tex <==
% \begin{table}[t!]
%     \centering
%     \begin{tabular}{|c|c|c|c|c|c|c|}\hline
%     &P& G&A&H&W&R\\\hline
%     P&&0.53&0.41&0.51&0.48&0.42\\\hline
%     G&0.53&&0.54&0.80&0.80&0.36\\\hline
%     A&0.41&0.54&&0.60&0.63&0.26\\\hline
%     H&0.51&0.80&0.60&&0.83&0.34\\\hline
%     W&0.48&0.80&0.63&0.83& &0.32\\\hline
%     R&0.42&0.46&0.26&0.34&0.32&\\\hline
%     \end{tabular}
%     \caption{\label{tab:correlation}Cosine similarity between different features in Pokec dataset (P-public, G-gender, A-age, H-heights, W-weight, R-region).}
%     \vspace{-0.3in}
% \end{table}    
\begin{table}[t!]
    \centering
    \begin{tabular}{|c|c|c|}\hline
    Pokec& Facebook&Pubmed\\\hline
    0.248&-0.01&0.107\\\hline
    \end{tabular}
    \caption{\label{tab:correlation} Pearson correlation between property feature and labels. }
    \vspace{-0.3in}
\end{table}    

% \begin{table}[t!]
%     \centering
%     \begin{tabular}{|c|c|c|}\hline
%     Pokec& Facebook&Pubmed\\\hline
%     0.53&0.92&0.94\\\hline
%     \end{tabular}
%     \caption{\label{tab:correlation}Cosine similarity between property features and classification labels. \Wendy{Measure Pearson correlation instead.}}
%     \vspace{-0.3in}
% \end{table}    


==> text/defense-dp.tex <==
\begin{figure*}[t!]
\centering
%   \vspace{0.1in}
    \centering
    \begin{subfigure}[b]{.6\textwidth}
      \centering
     \includegraphics[width=\textwidth]{text/figure/lap-defense-legend.pdf}
     \vspace{-0.2in}
    \end{subfigure}
    \begin{tabular}{cc}
    \begin{subfigure}[b]{.28\textwidth}
      \centering
     \includegraphics[width=\textwidth]{text/figure/gcn-embed1-dp.pdf}
     \vspace{-0.2in}
    \caption{\label{fig:gcn-dp-embed1} Attack $A^1_1$}
    \end{subfigure}
     \begin{subfigure}[b]{.28\textwidth}
      \centering
     \includegraphics[width=\textwidth]{text/figure/gcn-embed2-dp.pdf}
     \vspace{-0.2in}
    \caption{\label{fig:gcn-dp-embed2} Attack $A^2_1$}
    \end{subfigure}
    \begin{subfigure}[b]{.28\textwidth}
      \centering
     \includegraphics[width=\textwidth]{text/figure/gcn-post-dp.pdf}
     \vspace{-0.2in}
    \caption{\label{fig:gcn-dp-post} Attack $A_2$}
    \end{subfigure}
    \end{tabular}
    \vspace{-0.2in}
\caption{\label{fig:gcn-dp} Defense effectiveness of the Differential privacy defense method (GCN as the target model). \Wendy{merge with Figure 9. DP in dotted line.}}
% \vspace{-0.2in}
\end{figure*}

\begin{figure*}[t!]
\centering
%   \vspace{0.1in}
    \centering
    \begin{subfigure}[b]{.4\textwidth}
      \centering
     \includegraphics[width=\textwidth]{text/figure/classification-acc-legend(1).pdf}
     \vspace{-0.2in}
    \end{subfigure}
    \begin{tabular}{cc}
    \begin{subfigure}[b]{.27\textwidth}
      \centering
     \includegraphics[width=\textwidth]{text/figure/gcn-dp-acc-embed1.pdf}
     \vspace{-0.2in}
    \caption{\label{fig:gcn-dp-embed1-acc} Noise added to $Z^1$}
    \end{subfigure}
     \begin{subfigure}[b]{.27\textwidth}
      \centering
     \includegraphics[width=\textwidth]{text/figure/gcn-dp-acc-embed2.pdf}
     \vspace{-0.2in}
    \caption{\label{fig:gcn-dp-embed2-acc} Noise added to $Z^1 \& Z^2$}
    \end{subfigure}
    \begin{subfigure}[b]{.27\textwidth}
      \centering
     \includegraphics[width=\textwidth]{text/figure/gcn-dp-acc-post.pdf}
     \vspace{-0.2in}
    \caption{Noise added to posteriors\label{fig:gcn-dp-post-acc}}
    \end{subfigure}
    \end{tabular}
    \vspace{-0.2in}
\caption{\label{fig:gcn-dp-acc} Target model accuracy under the Differential privacy defense (GCN as the target model). \Wendy{Merge with Figure 10. DP in dotted line.}}
% \vspace{-0.2in}
\end{figure*}


==> text/defense-norm.tex <==
\begin{figure*}[t!]
\centering
%   \vspace{0.1in}
    \centering
    \begin{tabular}{ccc}
    \begin{subfigure}[b]{.27\textwidth}
      \centering
     \includegraphics[width=\textwidth]{text/figure/gcn-embed1-defense2.pdf}
     \vspace{-0.2in}
    \caption{\label{fig:gcn-norm-embed1}Embedding $Z^1$}
    \end{subfigure}
     \begin{subfigure}[b]{.27\textwidth}
      \centering
     \includegraphics[width=\textwidth]{text/figure/gcn-embed2-defense2.pdf}
     \vspace{-0.2in}
    \caption{\label{fig:gcn-norm-embed2}Embedding $Z^2$}
    \end{subfigure}
    \begin{subfigure}[b]{.27\textwidth}
      \centering
     \includegraphics[width=\textwidth]{text/figure/gcn-post-defense2.pdf}
     \vspace{-0.2in}
    \caption{\label{fig:gcn-norm-post}Posteriors}
    \end{subfigure}
    \end{tabular}
    \vspace{-0.2in}
\caption{\label{fig:gcn-norm-defense} The attack performance of Normalization for both black-box and white-box attack on GCN. }
% \vspace{-0.2in}
\end{figure*}

\begin{figure*}[t!]
\centering
%   \vspace{0.1in}
    \centering
    \begin{tabular}{ccc}
    \begin{subfigure}[b]{.27\textwidth}
      \centering
     \includegraphics[width=\textwidth]{text/figure/gcn-embed1-defense2-acc.pdf}
     \vspace{-0.2in}
    \caption{\label{fig:gcn-norm-embed1-acc}Embedding $Z^1$}
    \end{subfigure}
     \begin{subfigure}[b]{.27\textwidth}
      \centering
     \includegraphics[width=\textwidth]{text/figure/gcn-embed2-defense2-acc.pdf}
     \vspace{-0.2in}
    \caption{\label{fig:gcn-norm-embed2-acc}Embedding $Z^2$}
    \end{subfigure}
    \begin{subfigure}[b]{.27\textwidth}
      \centering
     \includegraphics[width=\textwidth]{text/figure/gcn-post-defense2-acc.pdf}
     \vspace{-0.2in}
    \caption{Posteriors\label{fig:gcn-norm-post-acc}}
    \end{subfigure}
    \end{tabular}
    \vspace{-0.2in}
\caption{\label{fig:gcn-norm-acc} Node classification performance after normalizing the embeddings and posteriors of GCN. }
% \vspace{-0.2in}
\end{figure*}

==> text/defense.tex <==
%\vspace{-0.1in}
\section{Defense Mechanisms}
\label{sc:defense}

% \Wendy{Add a paragraph explaining the intuition behind why adding noise on individual embeddings can defend against PIA.}

\subsection{Details of Defense Mechanisms}
%To countermeasure the privacy leakage of GPIA, we design two types of defense mechanisms for both black-box and white-box attacks respectively. Next, we present the details of these defense mechanisms.


{\bf Defense against black-box attacks.} As GPIA features are generated from the posteriors of the target model, we perturb these posteriors to defend against GPIA. In particular, for each node $v\in G$ and its associated posterior probabilities, 
 we add noise on each probability \cite{zhang2021inference} where the noise follows the Laplace distribution whose density function is given by $\frac{1}{2b} e^{ -\frac{x-\mu}{b}}$ ($b$: noise scale, $\mu$: the location parameter of the Laplace distribution). 
 %GPIA will be launched on the noisy posteriors. %\xiuling{$\frac{1}{2b} e^{ -\frac{x-\mu}{b}}$ is just a probability value of $x$, it means the variables of all the x should follow Laplace distribution, it isn't mean the amount of laplace noise, the amount of laplace noise is calculated in this way, firstly, calculate the cumulative distribution function of the inverse transform of laplace distribution, then laplace noise are generated by passing random uniform distributed variables to this cumulative distribution function.}
    
%        \item {\bf Top-k posterior output}: For each node $v\in G$, which is associated with $\ell$ posterior probability values, we keep the top-k largest posteriors. PIA will be launched on the {\em truncated} top-k posterior output. 
 %        \xiuling{\item {\bf Posterior normalization }: For each node $v\in G$, which is associated with $\ell$ posterior probability values, we use sigmoid function to normalize each value in $\ell$ to the range of (0,1).}
        
%    \item {\bf $D_3$: Classification label only} \xiuling{For each node $v_i$, we concatenate the classification label of each node in graph as the input of PIA model.  }

\input{text/defense-lap}
%  \input{text/defense-dp}
 \input{text/defense-trunc}
\input{text/defense-model-acc-gcn}

Besides the noisy posterior mechanism, we  evaluated two alternative methods: (1) {\em top-k posterior output} method: For each node $v\in G$ and its associated posterior probability values, we keep the top-k largest posteriors as the output. GPIA will be launched on the top-k posterior output; (2) {\em label-only output} method that the target model outputs the classification label instead of the posteriors. Our results show that both methods fail to either decrease GPIA accuracy significantly or provide acceptable target model accuracy. Thus we will not discuss these two defense mechanisms. 


{\bf Defense against white-box attacks.} We design two types of defense mechanisms that mitigate GPIA effectiveness by modifying the node embeddings: (1)  {\em  noisy embedding}: For each node $v\in G$, let $z$ be its node embedding. We add Laplace noise on $z$, where the noise follows the Laplace distribution whose density function is the same as noisy posterior method; and (2) {\em embedding truncation}: An embedding of dimension $d$ is converted to another embedding of lower dimension $d'= d\times (1-r)$, where $r\in(0, 1)$ is the {\em truncation ratio}. Higher $r$ indicates more dimensions to be truncated and less information is kept in the embedding. We randomly pick $d'<d$ dimensions from the original embedding.  Different node embeddings may have different dimensions to be truncated even under the same truncation ratio. 
 %   \item {\bf Embedding compression}: The intuition of embedding compression is to compress an embedding of dimension $d$ to another embedding of dimension $d'$, where $d'<d$. \Wendy{what's the objective function of compression, minimizing accuracy loss by compression?}
% We consider two types of embedding compression methods. Method 1 is straightforward. Given an embedding of dimension $d$, we keep the first  $[(1-r)\times d]$ elements in the embedding and remove the remaining, where $r\in(0,1)$ is the {\em compression ratio}. Higher $r$ leads to smaller dimension space after compression.  Method 2 first sorts the node’s embedding values in ascending order \Wendy{do you mean sort the values in each embedding, or do you mean sort all embeddings?}.  Then it keeps the the top $r\%$ percent of the sorted embedding as node’s new embedding, then we do max-pooling on each node’s new embedding, and concatenate the maximum value in each node’s new embedding as the embedding of graph, which is used as the input of PIA model. \Wendy{I don't think Method 2 is correct. It will bring huge loss in the qualify of the embedding. Can you try dimension reduction methods for Method 2?}
%  \xiuling{\item {\bf Embedding normalization }: For each node $v\in G$, let $z$ be its node embedding, we use sigmoid function to normalize each value in $z$ to the range of (0,1).}
  
%\end{ditemize}
For the embedding truncation method, we also implemented and evaluated three embedding dimension reduction methods including PCA \cite{minka2000automatic}, TSNE projection \cite{van2008visualizing}, and Autoencoder \cite{hinton2006reducing}. However, all of them fail to provide strong defense against GPIA, as they still preserve large amounts of information in the embedding which can be utilized by GPIA. Thus we will not present the details of these alternative truncation methods. 

\vspace{-0.1in}
\subsection{Evaluation of Defense Mechanisms}
We evaluate both effectiveness of the proposed defense methods and their impact on target model accuracy. We only consider attacks $A_1$ and $A_2$ as the defense effectiveness against these two attacks are expected to be applied to $A_3 - A_6$ due to their similarities. 

{\bf  Setup of defense mechanisms.} 
For both noisy embedding and noisy posterior defense mechanisms, we set the noise scale  $b=\{0.1,0.5,1,5,10\}$. For the embedding embedding truncation defense, we consider the compression ratio $r=\{0.01, 0.05, 0.1, 0.2, 0.3\}$. 
The setup of the target model is the same as in Section \ref{sc:exp-pia}. 

{\bf  Metrics.} We measure {\em defense effectiveness} as the accuracy of GPIA  against the GNN with defense, where attack accuracy is measured by Equation \ref{eqn:attacc}. 
We measure {\em target model accuracy} as the accuracy of node classification by the target model. 

%\xiuling{Finally, I don't use the accuracy of node classification by the target mode, because in that way, I need to have all the parameters (include weights and bias) of the original graphs, but I didn't save these parameters, if re-run the models, there are so many settings. 1000graphs*3gnns*6property task. So here I directly use the embbedings of layer1/layer2 to do node classification, i.e., the embeddings are directly fed into a MLP. The original node classification accuracy in figure 10 and 12 are also calculate in this way. It is much faster than re-train the gnns. Does it make sense? If doesn't make sense, I will re-run the GNNs.} \Wendy{No worries. Node classification by the target model is vague. I didn't give the details. }

{\bf  Baseline.} Differential privacy (DP) \cite{dwork2014algorithmic} has been shown as effective against inference attacks on ML models \cite{shokri2017membership,jayaraman2019evaluating}.  Therefore, we use differentially private deep learning method \cite{abadi2016deep} that adds Laplace noise to the gradients as the baseline. We set the noise scale $\epsilon=\frac{1}{b}$ (i.e., $\epsilon=$ \{10,5,1,0.5,0.1\}), where $b$ is the noise scale value for the noisy embedding/posterior scheme. Lower $\epsilon$ indicates stronger noise scale and thus strong privacy protection.  
 
{\bf  Effectiveness of defense.} We add the noise to the embeddings $Z^1$ and  $Z^2$ to defend against $A^1_1$ and $A^2_1$. We do not consider adding noise to both layers as more noise will lead to higher loss of target model accuracy. Figure \ref{fig:gcn-lap} shows the attack accuracy results under the noisy embedding/posterior defense when GCN is the target model. The defense performance on GraphSAGE and GAT are shown in Appendix \ref{appendix:gs-gat-defense1}. First, we observe that the noisy embedding/posterior defense can reduce the attack accuracy effectively by achieving the accuracy around 0.5 in all the settings. Second, different attacks require different amounts of noise to achieve the same degree of protection. For example, the defense against $A^1_1$ and $A^2_1$ requires the noise $b= 0.5$ and $b=5$ to reduce the attack accuracy  to be close to 0.5 respectively. Different properties also require different amounts of noise to be added to achieve the same degree of protection. For example, the defense against $A^2_1$ on $P_2$ and $P_5$ requires noise of scale $b=5$ and $b=0.5$ to reach the attack accuracy around 0.5. 
%\xiuling{The attack accuracy of the attacks can be reduced to close to 0.5 when $b\leq 0.5$ for $A_1^1$, $b<5$ for $A^2_1$ and $A_2$. }
%Furthermore, unsurprisingly, the defense power grows with the increase of the noise scale. In the white-box setting, the attack accuracy is decreased to 0.5 (random guess) when the noise scale reaches $b=1$ and higher. However, the defense method requires more noise (noise scale at least 5) to reduce the attack accuracy.

We also observe that the defense power of the DP baseline is weaker than our method in the defense against the white-box attack $A_1$ (Figure \ref{fig:gcn-lap} (a) \& (b)), even with the  noise scale as large as 10 (i.e., DP noise scale $\epsilon=0.1$). 
Indeed, similar observations have been made that DP is ineffective against GPIA for other target models such as HMMs and SVMs \cite{ateniese2013hacking}. 
Indeed, although DP provides theoretical guarantee of privacy protection against {\em individual data points}, it is unclear if it can provide sufficient protection over GPIA inference of aggregate information of a group of samples.  
Further, the data independence assumption of DP \cite{liu2016dependence} is indeed violated in the context of GNNs, as the edges in graph are dependent and correlated. However, we also observe that DP is effective against the black-box attack $A_2$ (Figure  \ref{fig:gcn-lap} (c)), and outperforms our method when the noise scale $b<5$ in most of the settings.  %it is because that the posteriors are perturbed after using DP, thus the distinguishability between graphs w/ or w/o property is reduced.  

Figure \ref{fig:gcn-trunc} (a) and (b) demonstrate the effectiveness of the embedding truncation defense method with GCN as the target model.  The defense performance on GraphSAGE and GAT are shown in Appendix \ref{appendix:gs-gat-defense2}.  The embedding truncation defense can reduce the attack accuracy of $A^1_1$ to be  close to 0.5 when the truncation ratio is as small as 0.1 (i.e., remove 10\% of embeddings).  However, it requires more noise (truncation ratio as large as 0.3) to reduce the attack accuracy of $A^2_1$ to be close to 0.5. We believe this is because $A^2_1$ is stronger than $A^1_1$ as it encodes more information in the embedding that can be utilized by the attack. 

{\bf Target model accuracy under defense.} 
We measure the GCN accuracy under the defense of the noisy posterior/embedding method, and show the result in  Figure \ref{fig:gcn-lap-acc}. The results of GraphSAGE and GAT are shown in  Appendix \ref{appendix:gs-gat-defense1}. First, unsurprisingly,  the target model accuracy downgrades when more noise is added to the embeddings/posteriors. The accuracy loss varies for different datasets. For example, the accuracy loss never exceeds 10\% for Facebook when the noise is added to $Z^2$, but becomes as large as 50.7\% for Pubmed dataset (Figure \ref{fig:gcn-lap-acc} (b)). Indeed, Pubmed dataset is the most sensitive to the defense among the three datasets, as it witnesses the largest amounts of accuracy loss. Second, the noisy embedding/posterior methods address the trade-off between privacy and accuracy well.  Target model accuracy remains to be acceptable when the defense is sufficient (i.e., the attack accuracy is reduced to close to 0.5). For example, for Pokec dataset,  when the noise scale $b=1$, the accuracy of attack $A_1^1$ has been mitigated to around 0.5 (Figure \ref{fig:gcn-lap} (a)), while the target model accuracy is 0.6 (Figure \ref{fig:gcn-lap-acc} (a)). 
Furthermore, the target model accuracy of our methods always outperforms that of DP baseline. This demonstrates that adding noise on embeddings and posteriors are better than adding noise on gradients in terms of the target model accuracy. 

We also measure the GCN accuracy under the defense of the  embedding truncation method, and show the result in  Figure \ref{fig:gcn-trunc} (c) \& (d). The results of GraphSAGE and GAT are shown in  Appendix \ref{appendix:gs-gat-defense2}. First, the target model accuracy downgrades with the increase of the truncation ratio, where the accuracy loss varies for different datasets and when different embeddings are truncated. For example, the target model accuracy loss is 13.9\% and 36.1\% for Facebook and Pubmed datasets respectively when $Z^1$ is truncated. Again,  Pubmed dataset witnesses the highest accuracy loss among the three datasets. Second, in terms of the trade-off between privacy and accuracy, the embedding truncation method loses to the noisy embedding method, as its target model accuracy is lower than that by the noisy embedding method under similar attack accuracy. For example, by the embedding truncation method, the target model accuracy is 0.58 for Facebook dataset (Figure \ref{fig:gcn-trunc} (d)) when the attack accuracy of $A^2_1$ against all properties becomes around 0.5 (Figure \ref{fig:gcn-trunc} (b)). This is slightly lower than that by the noisy embedding method, where the target model accuracy is 0.61 for Facebook dataset (noise scale $b=5$ in Figure \ref{fig:gcn-lap-acc} (b)) when the attack accuracy of $A^2_1$ against all properties becomes around 0.5 (noise scale $b=5$ in Figure \ref{fig:gcn-lap} (b)). 
%\Wendy{should emphasize target model accuracy is acceptable when the defense is strong enough.} \xiuling{But when the attack accuracy becomes 0.5, the target model accuracy is also very low. how about putting the embedding normalization performance here, the performance is much better I think }

% \Wendy{Add a paragraph with detailed results on diff between inference scores across different groups to explain why the defense works.}

\nop{
\xiuling{The attack performance of posterior normalization on GCN is shown in Figure \ref{fig:gcn-norm-post}, and the posterior quality after normalization is shown in Figure \ref{fig:gcn-norm-post-acc}. The defense performance and posterior quality on GraphSAGE and GAT are shown in Appendix \ref{appendix:gs-gat-defense4}. we observe that attack accuracy reduction is in the range of [13.1\%, 38.7\%]. The reason why the normalization defense approach can work is similar to embedding normalization that the posterior differences of between graphs with or without property become smaller. However, the posterior quality loss in terms of node classification accuracy is negligible, the classification accuracy difference of before and after normalization is less than 0.1\%. It is because that after normalization, the value order in the posterior of each node doesn't change, we think the node classification accuracy difference is caused by the randomness of node classification algorithm.} \Wendy{revise after the figure is updated.}
}


\nop{
\xiuling{The defense performance of \bf{Top-k posterior output} is shown in Table \ref{tab:topk}.} \xiuling{The results are not good, should it be removed?} \Wendy{removed.}
\begin{table}[t!]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \hline
     \multicolumn{2}{c|}{}&$P_1$&$P_2$&$P_3$&$P_4$&$P_5$&$P_6$\\ \cmidrule{1-8}
     \multirow{2}{*}{GCN}&before&0.99&0.99&0.99&0.88&0.8&0.92\\ \cmidrule{2-8}
    &after&0.99&0.99&0.99&0.89&0.8&0.91\\ \hline
     \multirow{2}{*}{GraphSAGE}&before&0.96&0.96&0.98&0.79&0.78&0.82\\ \cmidrule{2-8}
      &after&0.93&0.8&0.98&0.62&0.59&0.81\\ \hline
    \multirow{2}{*}{GAT}&before&0.9&0.91&0.96&0.79&0.71&0.84\\ \cmidrule{2-8}
    &after&0.88&0.81&0.96&0.64&0.61&0.81\\ \hline
    \end{tabular}
    \caption{Attack performance of \bf{Top-k posterior output} defense for black-box attack.}
    \label{tab:topk}
    \vspace{-0.2in}
\end{table}
}



==> text/discussion.tex <==
\section{Discussion}
\label{sc:discussion}

{\bf Extend to non-binary PIA models.}

{\bf Extend properties beyond nodes and links}

==> text/exp.tex <==
\section{Evaluation}
\label{sc:exp-pia}
%\xiuling{all the discussion part will be updated this afternoon and evening}
%To-do items for experiments
% 1. Target GNN of 3 layers. PIA with embeddings from layer 1, layer 2, layer 3, layer 1+2, Layer 2+3, layer 1+2+3
% 2. Attack performance of MLP, RF, and LF as GPIA classifier. Is there a winner among the three?
% 3. Node and edge importance and impacts on PIA
% 4. Defense performance
% 5. $A_5$ and $A_6$ performance on Pokec and Pubmed Datasets in Appendix

In this section, we aim to demonstrate the effectiveness of GPIA through answering the following three research questions:
\begin{ditemize}
    \item \textbf{RQ1} - How effective is GPIA on representative GNN models and real-world graph datasets?
\item{\bf RQ2} - Why GPIA work? 
\item{\bf RQ3} - How various factors (e.g., attack classifier models, embedding/posterior aggregation methods, and complexity of GNN models) affect GPIA effectiveness?
\end{ditemize} 
 

\begin{table}[t!]
    \centering
    \begin{tabular}{c|c|c|c|c}
    \hline
         \textbf{Dataset} & \textbf{\# nodes}  & \textbf{\# edges} & \textbf{\# features}  & \textbf{\#   classes}\\\hline
        %DBLP & 4501 & 6304 & 2 & 2 \\\hline 
        \textbf{Pokec} &45,036 & 170,964 & 5 & 2\\\hline
        \textbf{Facebook} &4,309 & 88,234 &1,284 & 2 \\ \hline 
        \textbf{Pubmed}  &19,717 & 44,338& 500 & 3\\\hline
    \end{tabular}
    \caption{Description of datasets}
    \label{tab:data}
    \vspace{-0.2in}
\end{table}
\nop{
\begin{table*}[t!]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}\hline
        Graph & \# of   nodes & \# of   Edges &\# of   Node features & Classification task / \# of   Classes& Properties to be attacked  / \# of   Classes\\\hline
         Pokec &45036 &170964 & 6&public / 2 &portion of male / 2\\\hline
         Pokec &45036 &170964 & 6&public / 2 &portion of (age > 20) / 2\\\hline
        %  Pokec &45036 &170964 & 6&public / 2 &portion of (age > 20) / 4\\\hline
        %  Pokec &45036 &170964 & 6&public / 2 &portion of (age > 20) / 8\\\hline
         Pokec &45036 &170964 & 6&gender / 2 &portion of (weight > 60KG) / 2\\\hline
         Facebook &4039 &88234 & 1284 &gender / 2 &portion of (educatiion type $\ge$ college) / 2\\\hline
         Pubmed &19717 &44338 & 500&paper type / 3 &portion of (appearance of word 'insulin') / 2\\\hline
    \end{tabular}
    \caption{Datasets and their properties to be attacked}
    \label{tab:data}
\end{table*}
}

\begin{table*}[t!]
    \centering
    \begin{tabular}{c|c|c|c|c}\hline
        \multirow{2}{*}{\bf Property} & \multirow{2}{*}{\bf Type} &\multirow{2}{*}{\bf Graph} & {\bf Property}  & \multirow{2}{*}{\bf Description} \\
         & & & {\bf feature} & \\\hline
        % $P_1$ & \multirow{3}{*}{Node-based} & Pokec &  Gender &  COUNT($v_\text{gender='Male'}$) $>$ COUNT($v_\text{gender='Female'}$)\\\cline{1-1}\cline{3-5}
        $P_1$ & \multirow{3}{*}{Node} & Pokec &  Gender &  \# of male nodes $>$ \# of  female nodes\\\cline{1-1}\cline{3-5}
        % $P_2 $ & & Facebook & Gender& COUNT($v_\text{gender='Male'}$) $>$ COUNT($v_\text{gender='Female'}$) \\\cline{1-1}\cline{3-5}
         $P_2 $ & & Facebook & Gender& \# of   male nodes $>$ \# of   female nodes \\\cline{1-1}\cline{3-5}
         %$P_3 $ & & Pubmed & keyword &   COUNT($v_\text{keyword = "Insulin"}$)> 0\\\hline
         $P_3 $ & & Pubmed & Keyword &  \# of publications with “IS” $>$ \# of publications without “IS”\\\hline\hline
         %$P_4 $ &\multirow{3}{*}{Link-based} & Pokec & {\em Gender} & COUNT($e_{v_i.\text{gender} = v_j.\text{gender}}(v_i, v_j)$) $>$ COUNT($e_{v_i.\text{gender} \neq v_j.\text{gender}}(v_i, v_j)$)\\         \cline{1-1}\cline{3-5}
         $P_4 $ &\multirow{3}{*}{Link} & Pokec & Gender & \# of   same-gender links $>$ \# of   diff-gender links \\
         \cline{1-1}\cline{3-5}
         %$P_5 $ & & Facebook & Gender & COUNT($e_{v_i.\text{gender} = v_j.\text{gender}}(v_i, v_j)$) $>$ COUNT($e_{v_i.\text{gender} \neq v_j.\text{gender}}(v_i, v_j)$)\\\cline{1-1}\cline{3-5}
         $P_5 $ & & Facebook & Gender & \# of   same-gender links $>$ \# of   diff-gender links\\\cline{1-1}\cline{3-5}
        %$P_6$ & & Pubmed & keyword (kw) &  COUNT($e_{v_i.\text{kw='IS'},  v_j.\text{kw='IS'}}(v_i, v_j)$) $>$ COUNT($e_{v_i.\text{kw='ST'},  v_j.\text{kw='ST'}}(v_i, v_j)$)
        $P_6$ & & Pubmed & Keyword  & \# of   citation links btw. papers with “IS” $>$ \# of   citation links btw. papers with “ST” \\\hline
    \end{tabular}
    \caption{Properties to be attacked by GPIA. same-gender (diff-gender, resp.) links indicate those links between users of the same (different, resp.) gender. “IS” = “Insulin”; “ST” = “Streptozotocin”. }
    \label{tab:property}
    \vspace{-0.1in}
\end{table*}


\subsection{Experimental Setup}
\label{sc:exp}

All the experiments are executed on Google COlab with Tesla P100 (16G) and 200GB memory. All the algorithms are implemented in Python with PyTorch. Our code and datasets are available online\footnote{https://anonymous.4open.science/r/PIA-CE14/}.

{\bf Datasets.}
We consider three real-world datasets, namely {\em Pokec}, {\em Facebook}, and {\em Pubmed} datasets, that are popularly used for graph learning in the literature: (1) {\bf Pokec} social network graph\footnote{https://snap.stanford.edu/data/soc-pokec.html} is collected from the most popular on-line social network in Slovakia. Nodes and edges in the graph represent the social network users and their friendship relationship respectively; (2) {\bf Facebook} social network graph\footnote{https://snap.stanford.edu/data/ego-Facebook.html}  consists of Facebook users as nodes and their friendship relationship as edges;  %Each node consists of the following features: birthday, education, work, name, location, gender, hometown, and language; 
and (3) {\bf Pubmed} Diabetes dataset\footnote{https://linqs-data.soe.ucsc.edu/public/Pubmed-Diabetes}  consists of 19,717 scientific publications from Pubmed database pertaining to diabetes that are classified into three classes. Each publication node is associated with 500 unique keywords (e.g., "cholesterol", "insulin", etc.) as well as the TF/IDF weight of these keywords as the features. The links between publications indicate the citation relationship. 
Table \ref{tab:data} summarizes the information of the three datasets. More details of the three datasets can be found in Appendix \ref{appendix:dataset}. 
The purpose of pick two graphs in one domain (social network graphs) and one graph from a different domain is for the validation of the effectiveness of transfer attacks ($A_3$ and $A_4$). 

{\bf Target GNN models.} 
We consider three state-of-the-art GNN models, namely GCN \cite{kipf2017semisupervised}\footnote{We use implementation of GCN at https://github.com/tkipf/pygcn}, GraphSAGE \cite{hamilton2018inductive} and GAT \cite{velickovic2018graph}\footnote{We use the implementation of both GraphSAGE and GAT from DGL package available at https://github.com/dmlc/dgl}, that are widely used by the ML  community. For each hidden layer, the number of neurons is 64, which is the same as the dimension of node embedding. We set the number of epoches for training as 1,500, and use early stop with the tolerance as 50. We set the dimension of node embeddings to 64 for all the three datasets. 

{\bf Properties.}  For each dataset, we design one node property and one link property to be attacked. The properties  are summarized in Table \ref{tab:property}. 
%The successful attacks on these properties can reveal the gender distribution information in Facebook and Pokec social network graphs, and the frequency distribution information of particular keywords (which can be sensitive) in Pubmed graph. 
We pick the keywords “Insulin” (IS) and “streptozotocin” (ST) for Pubmed dataset as they are the  keywords of the highest and lowest TF-IDF weight respectively. The successful attacks on these properties can reveal the gender distribution  in Facebook and Pokec social network graphs, and the frequency distribution of particular keywords (which can be sensitive) in Pubmed graph. 
We measure the impact of these properties on graph characteristics (node degree and node closeness centrality). The results can be found in Appendix \ref{sc:property-on-graph-char}. The main observation is that the presence/absence of these properties does not change the graph characteristics significantly. 
%Thus the property $P_6$ indicates if the training graph contains more citations between those publications with the most important keywords than the citations between those with the least important keywords. 


{\bf Implementation of attack classifier.} We use three types of attack classifiers for both attacks, namely Multi-layer Perceptron (MLP), Random Forest (RF), and Linear Regression (LR). 
We use the implementation of the three classifiers provided by sklearn package.\footnote{https://scikit-learn.org/}
We set up the MLP classifier of three hidden layers, with the number of neurons for each layer as 64, 32, 16 respectively. We use ReLU as the activation function for the hidden layers and Sigmoid for the output layer. We train 1,000 epochs with a learning rate of 0.001.  We use cross-entropy loss as the loss function and Adam optimizer.
For RF classifier, we set the maximum depth as 150 and the minimum number of data points allowed in a leaf node as 1. 
For LR classifier, we use the L2 norm as the penalty term, and liblinear\footnote{Liblinear libary: https://www.csie.ntu.edu.tw/~cjlin/liblinear/} as the optimization solver. We set the maximum number of iterations as 100 and the early-stop tolerance as 1e-4. 

{\bf Partial graphs.} We randomly sample 1,000 subgraphs from each dataset as the partial graph. The size of each partial graph is 20\%, 25\%, and 30\% of Pokec, Facebook, and Pubmed datasets respectively. 

{\bf GPIA training and testing data.} We randomly sample 1,000 subgraphs from each dataset to generate the training and testing data for GPIA. Each subgraph is of the same size as the partial graph. The training/testing split is 0.7/0.3, with the same number of positive and negative subgraphs in both training and testing data. 
% \Wendy{Explain the overlap between nodes and links in training and testing data.}
%For the other attacks ($A_3 - A_6$) that involve shadow graphs, we randomly sample shadow graphs in the same way as the partial graphs. 
%$\ShadowG$ and $\TargetG$ are orthogonal, and the node sizes of them are both half of original graph. Then we randomly sample 1000 subgraphs $\ShadowG_i$ from $\ShadowG$, 500 with property and 500 without property. Since we will test the dataset transferability here, we the node sizes of all $\ShadowG_i$ in all datasets are the same (we have explain the applicability in \ref{sc:white-attack}). The node sizes for  The training/testing split is 0.7/0.3, and the numbers of subgraphs with/without property are the same in training/testing data. Then we randomly sample 1000 subgraphs $\TargetG_i$ from $\TargetG$ as sub-target graphs, 500 with property and 500 without property. For $A_5$, $A_6$, we sample 1000 partial graphs $\PartialG_i$ from each dataset, the node size of each $\PartialG_i$ is the same as that of $\ShadowG_i$ in $A_3$ and $A_4$.  

 
{\bf Metrics.}  
We measure classification accuracy as the target model performance. 
We measure {\em attack accuracy} as the effectiveness of the proposed attacks.
In particular, 
\begin{equation}
\label{eqn:attacc}
\text{Attack accuracy} = \frac{N_c}{N},    
\end{equation}

where $N_c$ is the number of graphs that are correctly predicted by GPIA (either as positive or negative), and $N$ is the total number of graphs in the testing data. Intuitively, higher attack accuracy indicates that GPIA is more effective.

{\bf Baselines.} 
We consider three approaches as baselines for comparison with our GPIA model: (1)  {\bf Auxiliary summarization (Baseline-1)}: We adapt the {\em Directly Summarizing Auxiliary Dataset} (DSAD)  method \cite{zhang2021inference} to our setting as the baseline. %Due to the fundamental difference in the  properties considered by \cite{zhang2021inference} and ours, we modify DSAD approach by 
    We use a threshold of the average property values summarized from the adversary knowledge (e.g., partial graph) to predict the property of the target graph instead of training a classifier. We choose the threshold that has the best attack performance; (2) {\bf K-means clustering (Baseline-2)}: we apply k-means clustering on node embeddings and posteriors  where $k=2$. Then we measure the average distance between the centroid of each cluster to the embedding/posteriors by the target model on the target graph, and pick the cluster of the smaller distance; (3)  {\bf Meta-classifier (Baseline-3)}: We follow \cite{ateniese2013hacking,ganju2018property}  and use a  meta-classifier as the GPIA  classifier. 
    % \Wendy{Try the new baseline based on threshold of loss gap.}
    % \xiuling{My implementation is in this way: we averagely partition our GPIA training set to five parts, each parts has the same size of graphs with or w/o property, then we train five classifiers for each part, finally we feed the PIA testing data to each classifier and do majority voting of all the classifiers to get the final decision of whether the testing graphs are with or w/o property. }

%Specifically, for the white-box attack, given the node embedding of $N$ nodes from $l$th-layer of $\PartialG_i$, $Z_{i}^{l}_1, \dots, Z_{i}^{l}_N$, we firstly apply max-pooling to the all node embeddings, labeled as $Z^{'l}_{i}_1, \dots,Z^{'l}_{i}_N$, then we take the average value of $Z^{'l}_{i}_1, \dots,Z^{'l}_{i}_N$ as the feature value of  $\PartialG_i$. So for each $\PartialG_i$ in $\PartialG$, we will have a feature value and its label of w or w/o P. Then we try each feature value of $\PartialG_i$ as a threshold to predict whether a $\PartialG_i$ w or w/o P, and we select a threshold with best predict accuracy to predict whether a target graph w or w/o P.  \Wendy{How did you implement baseline for the black-box attack?}

% \subsection{Evaluation Results}
\input{text/pia-acc}

\subsection{GPIA Performance (RQ1)}

We launch the attacks $A_1$ - $A_6$ to attack GCN, GAT, and GraphSAGE, and measure their accuracy. To have a fair comparison of attack accuracy across different settings, we ensure that GPIA training data is of the same size for all the attacks.  We use RF and MLP as the white-box and black-box attack classifiers, max-pooling as the embedding aggregation method, concatenation as the posterior aggregation method, and TSNE projection as the embedding alignment method, as these setups produce the best attack performance. More results of the attack performance under different setups can be found in Section \ref{sc:att-settup}. As the possible hidden layers that the attacker collects node embeddings from is exponential to the number of hidden layers, we only consider GNNs of two hidden layers in this part of experiments to ease explanation. %We will show the effect of number of hidden layers to GPIA accuracy in Section \ref{sc:att-settup}. 

{\bf Performance of target GNN models.} Before we evaluate GPIA effectiveness, we evaluate the performance of the three GNN models, aiming to justify why they are worthy to be attacked. The performance of the three models can be found in Appendix \ref{appendix:gnn-performance}. First, all the three models perform well, with their classification accuracy significantly higher than the random guess. Therefore, these models are ready for the launch of GPIA. Second, the three models have good generalizability as the training-testing gap is in a small range of [0.02, 0.08]. Thus the three models do not have overfitting. 

{\bf Attacks $A_1$ and $A_2$.} 
For $A_1$, we consider six variants, namely those whose GPIA features are generated from  the embeddings at the first layer ($A_1^1$), at the second layer ($A_1^2$), at both first and second layers ($A_1^{1,2}$), and the aforementioned three cases together with the posteriors. 
We measured the performance of these variants, pick the best GPIA performance among all variants, and report it. More details of how the amounts of embeddings collected from different layers affect GPIA performance will be discussed in Section \ref{sc:att-settup}.

Figure \ref{fig:pia_acc} shows the results of the attack accuracy of our proposed attacks as well as the baseline methods. 
First, we observe that the attack accuracy of $A_1$ and $A_2$ ranges in [0.62, 1], which is significantly higher than 0.5 (random guess). In some settings (e.g., GCN target model and node properties in Figure \ref{fig:pia_acc} (a)), the attack accuracy can be as high as close to 1, even under the black-box setting. This demonstrates the effectivenss of GPIA against these target models. 
Furthermore, the accuracy of $A_1$ and $A_2$ are much higher than Baseline-1 and Baseline-2, which is close to 0.5. In addition,  the performance of $A_1$ and $A_2$ is similar to Baseline-3. In other words, using either one classifier or stacking multiple classifiers into a meta-classifier does not impact the GPIA performance. 

Second, although the attack performance varies across different types of properties, the attack accuracy of GPIA against the three node properties ($P_1$ - $P_3$) is noticeably higher than the link properties ($P_4$ - $P_6$) in general. The only exception is for the property $P_6$ and GAT as the target model (Figure \ref{fig:pia_acc} (c)), where the attack accuracy of $P_6$ is close to that of $P_3$, and higher than $P_1$ and $P_2$. One possible reason that GPIA is more successful against the node properties than the link properties is that it only needs to infer the node feature distribution over node features, but it has to infer both node feature distribution and graph structure for the link properties.  

Third, we observe that the accuracy of the white-box and black-box attacks is very close. The difference between them is negligible in most of the cases. 
%\footnote{The difference between the white-box and black-box attacks exceeds 0.1 in only few cases}. 
Interestingly, the white-box attack does not always outperform the black-box attack,  even though its features may include those features used by the black-box attack, possibly due to overfitting of the GPIA classifier by including more features. 
This demonstrates the power of the property inference - the black-box access to the target model is sufficient to launch the attack. 

%Third, we observe that the attack always performs worse on GAT than GCN and GraphSAGE, it is because that GAT uses the attention mechanism to aggregate the feature information of neighbor nodes, the attention mechanism will aggregate neighbor nodes with different attention scores. While GCN and GraphSAGE aggregate all the neighbor nodes with same weights.  For GCN and GraphSAGE, we don’t detect significant difference in terms of the attack accuracy of white-box attack ($A_1^1$ and $A_1^2$), although GraphSAGE aggregates the node feature information over randomly sampled neighbors. Actually, in our experiments, we find that the white-box attack accuracy of GraphSAGE is much lower than GCN when we use the “concatenation” approach to generate the graph embedding which will then feed to the attack model (the white-box attack accuracy with concatenation of GCN can be found in Figure \ref{fig:dif-ft}, and that of Graphsage can be found in Figure  \ref{fig:dif-ft-gs-gat}.) It also indicates the effectiveness of our max-pooling approach. And we observed that the black-box attack accuracy of GraphSAGE is lower than GCN, it is because GraphSAGE aggregates the node feature information over randomly sampled neighbors, which will preserve less information of graph compared with GCN. \Wendy{To-do: The discussion may need to be revised after the white-box attack results are updated.}


 


\input{text/attack34-acc}
\input{text/attack56-acc}

{\bf Attacks $A_3$ and $A_4$.} Figure \ref{fig:attack34-acc} presents the results of $A_3$ and $A_4$. The results of GAT and GraphSAGE models are included in Appendix \ref{appendix:attack34-gs-gat}. In all the settings,  $A_3$ and $A_4$ are effective as their accuracy is higher than 0.5 (random guess). The attack accuracy can be as high as 0.66 when the adversary uses the Facebook social network graph as the shadow graph to infer whether the Pokec social network graph has disproportionate distribution between male and female users. In other words, GPIA can transfer the knowledge learned from a graph to infer the properties of another graph. 
However, the accuracy of both $A_3$ and $A_4$ is worse than $A_1$ and $A_2$. This is not surprising as both $A_3$ and $A_4$ learn the knowledge from the shadow graph whose data distribution can be different from the target graph. We also observe that GPIA sometimes performs better under the settings that shadow and target datasets belong to different domains than the settings that they belong to the same domain.  For example, as shown in Figure \ref{fig:attack34-acc} (a), GPIA accuracy can be as high as 0.71 when Pubmed and Pokec datasets are the target and shadow datasets respectively, but it is only 0.66 when the target dataset is changed to Facebook dataset while keeping Pokec dataset as the shadow dataset, although both Pokec and Facebook datasets are social network graphs. We analyze the reason behind this observation, and found Pokec and Facebook datasets have different graph characteristics in terms of node degree and node closeness centrality, although they are from the same domain.  %\xiuling{maybe we can list more graph characteristic here, such as graph density, modularity, etc }. 
Indeed, Pubmed dataset is more similar  to Pokec dataset than Facebook dataset in terms of node degree and node closeness centrality. More details of the graph characteristics of the three datasets can be found in Table \ref{tab:graph-charact} in Appendix. 
Furthermore, the data distribution in Facebook and Pokec datasets are less similar than that between Pubmed and Pokec datasets, which leads to smaller attack accuracy. 
% \Wendy{Add explanation of why A3/A4 have attack accuracy lower than 0.6 in many cases, but "using an attack model trained on Pubmed gives nontrivial performance on Facebook/Pokec". Add experimental results of loss-gap between training and testing data (similar to the new results in Response).}
%We analyze the reason behind this observation. We found that Pokec and Facebook datasets have different graph characteristics, although they are from the same domain. Indeed, Pubmed dataset has more similar graph characteristics in terms of node degree and node closeness centrality to Pokec dataset than Facebook dataset. The graph characteristics of the three datasets can be found in Appendix \ref{sc:graph-chacteristics}. \Wendy{Besides graph characteristics, also need to study the data distribution on the property features for three different graphs. One way to do this to measure the percentage of males and females in Facebook and Pokec datasets, and the percentage of IS in Pubmed dataset}




{\bf Attacks $A_5$ and $A_6$.} We vary the portions of $\ShadowG$ and $\PartialG$ in the adversary knowledge when we evaluate the effectiveness of $A_5$ and $A_6$. 
Figure \ref{fig:attack56-acca-pokec-fb} present the attack accuracy result of both properties $P_1$ (node property) and $P_4$ (link property) with the partial graph  sampled from Pokec dataset and the shadow graph sampled from Facebook dataset. Note that both Pokec and Facebook are social network graphs. 
The performance of other settings are shown in Appendix \ref{appendix:attack56-2}. 
We have the following observations. First,  the accuracy of $A_5$ and $A_6$ in all the settings is higher than 0.5, i.e., both attacks are effective. Furthermore, the attack accuracy increases as the size of the partial graph grows. In particular, when the partial graph size dominates the shadow graph size (e.g., when the ratio exceeds 4:1),  the attack accuracy against the property $P_1$ can be close to 1 for both $A_5$ and $A_6$ for GCN model, and no less than 0.7 for GAT and GraphSAGE. 
Second, the attack accuracy of $A_5$ and $A_6$ on $P_1$ is lower than that of the attacks $A_1$ and $A_2$ (i.e., only the partial graph is available), similarly for $P_4$. This is because the features collected from the shadow graphs may not be consistent with that of the partial graph, and indeed degrade GPIA performance.  
On the other hand, the attack accuracy of $A_5$ and $A_6$ is higher than that of $A_3$ and $A_4$. This is unsurprising as, compared with $A_3/A_4$, $A_5$ and $A_6$ utilizes the additional knowledge learned from the partial graph to improve its accuracy. 


%{\bf Main Takeaways.} GPIA is effective on all six attacks. In particular, its performance on $A_1$ and $A_2$ is superior to Baseline-1 and Baseline-2, and similar to Baseline-3.  The attack against node properties performs better than that against link properties. The white-box and black-box attack performance are similar in $A_1$ and $A_2$. GPIA is less effective on $A_3$ and $A_4$ compared to $A_1$, $A_2$, however the performance is superior to random guess. The attack performance of $A_5$ and $A_6$ is higher than that of $A_3$, $A_4$ but less than $A_1$, $A_2$. When the dominance of $\PartialG$ increases, the performance of $A_5$ and $A_6$ increases. 

% \Wendy{Add new results of training \& testing data without overlap (Reviewer R3).}

\Wendy{Add new results of sparse graph}

\vspace{-0.2in}
\subsection{Why GPIAs Work? (RQ2)} 
As the experimental results have demonstrated the effectivenss of GPIA, next, we analyze why GPIAs can infer the existence of property in the training graph successfully. Conducting the theoretical analysis is very challenging due to the complexity in both training data and GNN models. Thus we discuss why GPIAs work based on practical evaluations.

% \Wendy{Add a paragraph titled "Group (im)balance". Add evaluation of various group ratios: 1:1, 1:2, 1:4. }

{\bf Correlation between property features and labels.} One possible factor that contributes to GPIA's success is that there exists a strong correlation between the property feature and the class label, which makes the target model's behaviors rely heavily on the property feature so that they vary significantly for positive and negative graphs. Following this, we measure the Pearson correlation between the property feature and class label of the three graph datasets. It turns out that all the three graphs have weak Pearson correlations between the property feature and the label; the Pearson correlation value is 0.248, -0.01, and 0.107 for Pokec, Facebook, Pubmed datasets respectively. This shows that the correlation between property feature and class label doe not play an important role in the success of GPIA.  
% \Wendy{Add the sentence: "Since the correlation between property features and labels does not contribute to GPIA's success, the leakage is not an artifact of the model".}

{\bf Overfitting.} Previous work \cite{shokri2017membership} has shown that overfitting is a major factor that causes a model to be vulnerable to membership inference attacks. However, it is not clear whether overfitting of target classifiers has any role in the property inference attack. In our case, all the three GNN models have good generalizability (shown in Appendix \ref{appendix:gnn-performance}). We plan to study the relationship between overfitting and property inference in more detail in the future. 

{\bf Disparate influence across different groups.} As observed by the recent studies, ML models are “biased” in the sense that they behave differently across different groups in the training data  \cite{chouldechova2018frontiers,pessach2022review}. Such group bias make the GNN models behave differently on positive and negative graphs, which can be utilized by GPIA for inference. Following this, we measure the disparity in GNN model accuracy  across different node groups in Facebook and Pokec datasets. The results are included in Appendix \ref{appendix:disparity}. We observe the existence of accuracy disparity to some extent for all the three GNN models. In particular, the disparity is significant on Facebook dataset, where the difference in node classification accuracy across male and female groups can be as large as 0.13. 
The disparity demonstrates that the GNN models behave differently for different node/link groups. Such different behaviors lead to the dissimilarity in embeddings/posterior distribution for positive and negative graphs where  different groups dominate the data. Such dissimilarity can be picked up by GPIA to learn and infer. 
%We will further investigate the relationship between fairness and GPIA in the future. 

To have a deeper understanding of GNN models' behaviors towards different node/link groups, we measure the {\em influence score} of individual node/link to quantify the impact of a node/link on the GNN model performance. An intuitive idea measuring the influence of a given training node/link on a GNN model is to ask the counterfactual~\cite{feldman2020does,koh2017understanding}: {\em what would happen to the model behaviors if the model did not see the node/link}? Answering this counterfactual enables to connect the model's behaviors with the training data.

To quantify the effect of the counterfactual, we measure the difference in the model behaviors when it is trained with and without a particular node/link. We use gradients to capture the model behaviors. Formally, assuming %$\theta_{v}\stackrel{\Delta}{=}\TargetM(\TargetG\backslash\{v\})$,
$\g_{v}\stackrel{\Delta}{=}\nabla\mathcal{L}(\TargetG\backslash\{v\})$, 
that is, $\g_{v}$ is the set of gradients induced from the training of  the target model $\TargetM$ given the graph $\TargetG$ excluding the node $v$, where $\mathcal{L}$ is the loss function of $\TargetM$. 
Then the {\em influence score of a node $v$} on $\TargetM$ is measured as 
\[I(v)\stackrel{\Delta}{=}distance(\g_{v}, g),\] where $g$ is the set of gradients induced by $\TargetM$ on $\TargetG$. Intuitively, higher influence score indicates the node $v$ impacts more on $\TargetM$. Similarly, %assuming $\theta_{e}\stackrel{\Delta}{=}\TargetM(\TargetG\backslash\{e\})$ 
assuming $g_{e}\stackrel{\Delta}{=}\nabla\mathcal{L}(\TargetG\backslash\{e\})$ for a given edge $e\in G$, the {\em influence score of an edge $e$} on $\TargetM$ is measured as 
\[I(e)\stackrel{\Delta}{=}distance(g_{e}, g).\]
Various distance functions (e.g., Euclidean distance and cosine similarity) can be used. We use cosine similarity as the distance function. After we compute the influence score of individual nodes and links, we compute the average influence score of nodes/links in a particular group as the influence score of the group.

% \Wendy{Evaluate loss of each group in training and testing data, and measure the gap. Add this in Table 6.}

We consider the properties $P_2$ and $P_4$ of Facebook dataset, and  compute the average influence score for male and female node groups (group by $P_2$), as well as the same-gender and diff-gender links (group by $P_4$). The results of influence scores are reported  in Table \ref{tab:inf-score}. We observe that all GNN models have noticeable disparity in the influence scores across different groups. For example, the influence scores of the female group is less than half of that of the male group for GCN. This aligns with our hypothesis: \emph{different node/link groups have different influence on GNN models}, and thus, enables GPIA to distinguish positive and negative graphs where different node/link groups dominate these graphs. 
%However, which group has higher influence scores varies for different GNN models. For example, the male node group has higher node influence score for both GCN and GraphSAGE, but lower score for GAT. 

\begin{table}[t!]
    \centering
    \begin{tabular}{c|c|c|c|c}
    \hline
     \multirow{2}{*}{{\bf GNN model}}&\multicolumn{2}{c|}{{\bf Node groups}}&\multicolumn{2}{c}{{\bf Link groups}}  \\ \cline{2-5}
     &Male&Female&Same-gender&Diff-gender\\ \cline{1-5}
     GCN&0.038&0.017&0.022&0.012\\ \cline{1-5}
     GraphSAGE&0.022&0.015&0.0039&0.011\\ \cline{1-5}
     GAT&0.057&0.087&0.034&0.03\\ \hline
    \end{tabular}
  \caption{Influence scores of different node/link groups (Facebook dataset). }
    \label{tab:inf-score}
    \vspace{-0.2in}
\end{table}

\nop{
\subsection{Why PIAs Work (RQ2)?}
As the experimental results have demonstrated the effectivenss of GPIA, next, we analyze why PIA can infer the existence of property in the training graph successfully. Conducting the theoretical analysis of why PIA can work is very challenging due to the complexity in both training data and GNN models. Thus we discuss why PIAs work based on practical evaluations.  

\input{text/p-feature-impact}
\input{text/distriution-pokec}

%\input{text/post-diff-tsne}

%\xiuling{Figure \ref{fig:post-diff-gcn} illustrates the distribution of element-wise difference in posterior probability for graphs with or w/o property. We can observe the distinguishability of graphs with or w/o property by using element-wise difference, this is why we use the element-wise difference approach in Section \ref{sc:black-box-ttack}. }

%{\bf Distribution of average  difference in posterior probability by the target model with vs w/o property}  

{\bf GPIA Independence from correlation between property feature and class label.} One possible factor that contributes to GPIA's success is that there exists a strong correlation between the property feature and the class label. Such correlation can make the target model rely heavily on the property feature and thus its output varies significantly for positive and negative graphs. To validate this, we measure the Pearson correlation between the property feature and class label of the three graph datasets. However, it turns out that all the three graphs have weak Pearson correlations between the property feature and the label; the Pearson correlation value is 0.248, -0.01, and 0.107 for Pokec, Facebook, Pubmed datasets respectively. This shows that the correlation between property feature and class label doe not play an important role in the success of GPIAs. 

{\bf Data distribution of property features on target model.} Although there does not exist a strong correlation between the property feature and class label, the property feature may still impact the target model in the way that different data distributions on the property features change the target model output. To formalize such impact, we ask the counterfactual: {\em what would the target model behave if the values of the property feature were changed}? Note that changing the value of the property feature can change the graph from positive (negative, resp.) to negative (positive, resp.) consequently.  
To answer this question, we generate a number of pairs of positive and negative graphs that have the same graph structure but only differ at the property feature. 
In particular, given a graph $\TargetG$, we generate its {\em reverse} version $\bar{\TargetG}$ so that $\TargetG$ and $\bar\TargetG$ have the same graph structure but opposite property states, i.e., $\bar\TargetG$ is negative (positive, resp.) if $\TargetG$ is positive (negative, resp.). 
For both node properties $P_1$ and $P_2$ (on Pokec and Facebook graphs), we generate $\bar\TargetG$ by flipping the values on their property feature (i.e., change male/female to female/male). While for both link properties $P_4$ and $P_5$ on these two graphs, we generate $\bar\TargetG$ by converting the same-gender edges into diff-gender ones and the diff-gender edges into same-gender ones via changing the gender value. 
For both properties $P_3$ and $P_6$ on Pubmed graph, we generate $\bar\TargetG$ by flipping the  keywords “Insulin” with “Streptozotocin”. 
%\xiuling{For $P_3$, $\bar\TargetG$ is also generated by flipping the values on their property feature (i.e., whether the TF/IDF value is 0)}
%Finally, for $P_6$ on Pubmed graph, we generate $\bar\TargetG$ by switching the keywords “Insulin” and  “Streptozotocin”. 
%For Property $P_3$ on Pubmed graph, we generate $\bar\TargetG$ by re-setting the TF/IDF value of  keywords “Insulin”, if the original TF/IDF value is 0, we reset it as a random non-zero value in (0,1], otherwise, we reset it as 0. For both properties $P_4$ and $P_5$ (on Pokec and Facebook graphs), we generate $\bar\TargetG$ by converting some of the same-gender edges into diff-gender ones or converting diff-gender edges into same-gender ones via changing the gender value to guarantee $\TargetG$ and $\hat{\TargetG}$ have different property. }
Next, we run the same GNN model on both $\TargetG$ and $\hat{\TargetG}$, and measure the distance between node embeddings and posterior outputs generated from them. 
To measure the distance of node embeddings, we follow \cite{hinton2002stochastic} to transfer the node embeddings into a probability distribution based on the scaled squared Euclidean pairwise distance between node embeddings. Then we use Jensen-Shannon divergence (JSD) \cite{majtey2005jensen} to measure the distance between the two probability distributions from $\TargetG$ and $\bar\TargetG$. 
%The distance between node embeddings is measured as the average Euclidean distance between embeddings 
%\begin{equation}
%Dis=\frac{\sum_{\forall v_i\in\TargetG}Euclidean(z_i, z_i')}{|V|},    
%\end{equation}
%where $z_i$ and $z_i'$ are the embedding of the node $v_i$ generated from $\TargetG$ and $\bar\TargetG$ respectively. 
The distance between posterior outputs is measured as JSD between the two posterior output distributions. The JSD distance is within the range [0, 1], where smaller value indicates the closer distributions. Finally, for each dataset, we generate 1,000 pairs of positive and negative graph pairs for node properties ($P_1$ - $P_3$) and 100 pairs for link properties ($P_4$ - $P_6$), and compute the average JSD distance of these pairs. 

We report the results of average JSD distance between embeddings/posteriors across positive and negative graphs in Table \ref{tab:compare1}. We observe although the distance varies for different target models and properties, there exists noticeably large JSD distance in many settings. The distance can be as large as 0.56 ($P_3$ with $Z^1$ and GraphSAGE). There are only 7 out of 54 settings whose JSD distance is less than 0.15. This demonstrates that the data distribution on the property feature have substantial influence on the behaviors of the target model, and thus explains why PIA can work. 

%{\bf Main Takeaways.} \Wendy{add summary of why $PIA$ works.} \xiuling{PIA works because the embedding/posterior distribution between graphs w/ or w/o property are highly distinguishable. The cause of this kind of distinguishability is that the distribution of property feature in a graph has significant impact on the distribution of embeddings and model outputs.   }

{\bf Distinguishable distribution of embeddings/posteriors from positive and negative graphs.} Intuitively, GPIA can predict the presence of the property because the output (either node embeddings or posteriors) of the positive a and negative graphs are distinguishable. To validate this, first, we compare the distribution of graph embeddings and posteriors generated from positive and negative graphs. Figure \ref{fig:dis_pokec} illustrates the distribution of both graph embedding and posteriors generated by GCN model on a pair of positive and negative graphs sampled from Pokec graph. We ensure both graphs only differ on their property feature. 
First, for the node property (Figure \ref{fig:dis_pokec} (a) - (c)), both node embeddings and posteriors from positive and negative graphs are well separated. Furthermore, node embeddings from the negative graph (red dots) are closer to each other than those (blue dots) from the positive graph. This also applies to the posteriors. This enables PIA to predict the property $P_1$ by utilizing the distance between node embeddings and posteriors. Second, for the link property (Figure \ref{fig:dis_pokec} (d) - (e)),  embeddings and posteriors do not show the same well-separateness pattern as the link property. However, node embeddings from the positive graph (blue dots) are closer to each other than those (red dots) from the positive graph. Thus GPIA is able to predict the presence of $P_4$ in Pokec dataset, but with a lower GPIA accuracy than the property $P_1$ (as shown in Figure \ref{fig:pia_acc} (a)). 
We have similar observations for both GAT and GraphSAGE models; more details can be found in Appendix \ref{appendix:dis_pokec2}. 
}

\subsection{Factors Impacting GPIA performance (RQ3)}
\label{sc:att-settup}

In this section, we investigate how various factors impact GPIA performance. We consider the following factors, including the type of attack classifier model, the type of embedding /posterior aggregation methods, the type of dimension alignment methods, and the complexity of GNN models. 
We also consider the impact of the amounts of embeddings collected from different layers of the GNN models on GPIA, and observe that GPIA performance stays stable for all possible settings. The results are included in Appendix \ref{appendix:multi-ft2}.

% \begin{table}[t!]
%     \centering
%     \begin{tabular}{c|c|c|c|c|c|c|c}
%     \hline
%      \multicolumn{2}{c|}{Attack classifier} & $P_1$ & $P_2$& $P_3$& $P_4$& $P_5$& $P_6$  \\ \hline
%      \multirow{3}{*}{$A_1^1$}&MLP&{\bf 0.98}&{\bf 0.96}&{\bf 0.82}&0.9&0.64&0.63\\\cmidrule{2-8}
%      &RF&{\bf 0.98}&{\bf 0.96}&{\bf 0.82}&{\bf 0.91}&{\bf 0.65}&{\bf 0.65}\\\cmidrule{2-8}
%      &LR&0.95&0.95&0.8&0.62&0.63&0.63\\\hline
%         \multirow{3}{*}{$A_1^2$}&MLP&{\bf 0.97}&{\bf 1}&0.94&0.85&0.77&0.78\\\cmidrule{2-8}
%         &RF&{\bf 0.97}&{\bf 1}&{\bf 0.96}&{\bf 0.86}&{\bf 0.78}&{\bf 0.82}\\\cmidrule{2-8}
%         &LR&0.92&0.99&0.93&0.6&0.77&0.72\\\hline
%         \multirow{3}{*}{$A_2$}&MLP&{\bf 0.99}&{\bf 1}&{\bf 0.99}&0.87&{\bf 0.83}&{\bf 0.93}\\\cmidrule{2-8}
%          &RF&{\bf 0.99}&0.99&{\bf 0.99}&{\bf 0.88}&0.82&0.92\\\cmidrule{2-8}
%         &LR&{\bf 0.99}&0.98&{\bf 0.99}&0.83&0.73&0.89\\\hline
        
%         % \multirow{3}{*}{MLP}&$A_1^1$&0.98&0.96&0.82&0.9&0.64&0.63\\\cmidrule{2-8}
%         % &$A_1^2$&0.97&1&0.94&0.85&0.77&0.78\\\cmidrule{2-8}
%         % &$A_2$&0.99&1&0.99&0.87&0.83&0.93\\\hline
%         % \multirow{3}{*}{RF}&$A_1^1$&0.98&0.96&0.82&0.91&0.65&0.65\\\cmidrule{2-8}
%         % &$A_1^2$&0.97&1&0.96&0.86&0.78&0.82\\\cmidrule{2-8}
%         % &$A_2$&0.99&0.99&0.99&0.88&0.82&0.92\\\hline
%         % \multirow{3}{*}{LR}&$A_1^1$&0.95&0.95&0.8&0.62&0.63&0.63\\\cmidrule{2-8}
%         % &$A_1^2$&0.92&0.99&0.93&0.6&0.77&0.72\\\cmidrule{2-8}
%         % &$A_2$&0.99&0.98&0.99&0.83&0.73&0.89\\\hline
%     \end{tabular}
%     \caption{Impact of type of attack classifiers on GPIA performance. The best attack accuracy for each attack setting is highlighted in bold. \Wendy{Add results of $A_1^{1,2}, A_1^{1,2,o}$. change to bar type.}}
%     \label{tab:impact-classifier}
%     \vspace{-0.2in}
% \end{table}
\input{text/impact-classifier}
{\bf Type of attack classifier models.} 
We measure GPIA accuracy when MLP, RF, and LR are used as the attack classifiers, and include the results in Appendix \ref{appendix:pia-classifier-graphsage-gat} due to the limited space. 
%The results on GraphSAGE and GAT are shown in Appendix \ref{appendix:pia-classifier-graphsage-gat}. 
The main observation is that, while the three attack classifiers deliver similar performance in most of the settings, LR never outperforms MLP and RF. Furthermore, RF outperforms MLP slightly in  most of the white-box attacks,  while  MLP has slightly better performance than RF for the  black-box attacks.  Therefore, we recommend RF and MLP as the white-box and black-box attack classifier respectively. 
%\input{text/agg-comp}
\input{text/more-layers} 

\nop{
\begin{figure}[t!]
    \centering
%   \vspace{0.1in}
      \centering
    %  \includegraphics[width=\textwidth]{text/figure/gcn-pia.pdf}
    \includegraphics[width=0.3\textwidth]{text/figure/agg-post-legend(1).pdf}\\
    \includegraphics[width=0.25\textwidth]{text/figure/gcn-post-agg.pdf}
     \vspace{-0.1in}
    % \caption{GCN}
\caption{\label{fig:dif-ft-posterior-aggregation} Impacts of posterior aggregation method (element-wise difference) on GPIA performance (GCN as target model). } 
 \vspace{-0.1in}
\end{figure}
}
%\input{text/attack34-compare}
%\input{text/more-paras}

{\bf Embedding/posterior aggregation methods.} We measure the impacts of the three embedding aggregation methods (i.e., concatenation, max-pooling and mean-pooling) on GPIA performance, and include the results in Appendix \ref{appendix:agg-embedding-graphsage-gat} due to the limited space. 
%Figure \ref{fig:dif-ft-embedding-aggregation} shows the results when GCN is the target model. The results of GraphSAGE and GAT models can be found in Appendix \ref{appendix:agg-embedding-graphsage-gat}. 
The main observation is that max-pooling outperforms the other two methods in most of the settings. Therefore, we recommend  max-pooling as the embedding aggregation method.

We also measure the impact of two different posterior aggregation methods, namely concatenation and element-wise difference, on GPIA. Our main observation is that the concatenation method always lead to either equal or slightly better GPIA performance than element-wise difference. 
%Figure \ref{fig:dif-ft-posterior-aggregation} shows the results  when GCN is used as the target model. The results on GraphSAGE and GAT models are similar and can be found in Appendix \ref{appendix:agg-posterior-graphsage-gat}. 
Due to limited space, we include the results in Appendix \ref{appendix:agg-posterior-graphsage-gat}. 


{\bf Dimension alignment methods.}
We measure GPIA performance for the four alignment methods, namely, sampling, TSNE projection, PCA dimension reduction, and Autoencoder compression, on the three target models. 
We put the results in Appendix \ref{sc:pca-encoder-acc} due to the limited space. 
%Table \ref{tab:attack34-compare} presents the results of the attack accuracy under different dimension alignment methods when GCN is the target model and GPIA is launched against the node-level properties. 
%The results of with GraphSAGE and GAT as target model are shown in Appendix \ref{sc:pca-encoder-acc}. 
The results suggest using TSNE as the dimension alignment method, as it delivers the best attack accuracy. On the other hand, the Autoencoder method always delivers the worst GPIA accuracy among all four alignment methods. 
%\xiuling{Table \ref{tab:attack34-compare} show the performance of white-box attack ($A_3^1$) with different dimension alignment methods, do we need to show the performance of $A_3^2$ and black-box attack with different dimension alignment methods here? If we put $A_3^2$ and black-box attack of GCN, $A_3^1$,$A_3^2$ and black-box attack of GraphSAGE and GAT in appendix, it will include 8 table in Appendix, so which settings we should show in Appendix.}





%First, the attack with embeddings from $2^{nd}$-layer ($A_1^2$) not always outperforms the attack with embeddings from $1^{st}$-layer ($A_1^1$), \xiuling{and embeddings from $3^{rd}$-layer ($A_1^3$) not always outperforms the attack with embeddings from $1^{st}$-layer ($A_1^1$) or $2^{nd}$-layer ($A_1^3$), which is consistent with the observations of Figure \ref{fig:more-layers}}. It is because that although the embeddings from $2^{nd}$-layer aggregate more node features (the features of both 1-hop and 2-hop neighbor node) than the embeddings from $1^{st}$-layer (only aggregate the node features of 1-hop neighbor nodes), aggregating features from larger number of nodes results in higher averaging (over-smoothing of features), which will reduce the  distinguishability of features \cite{li2018deeper}.  \Wendy{The discussion needs to be revised. It cannot be about $Z^1$ and $Z^2$ only. You should also discuss the cases with embeddings from 2 layers and 3 layers. } \xiuling{Second, we observe that the feature that combining more embeddings from different layers not always outperform that of single layer embeddings, it is because that the embeddings distribution from different layers are different, the combination of embeddings from different layers may bring more noisy sample to the original feature (single layer embeddings), thus worsen the attack performance. }



{\bf Complexity of GNN models.} 
We define the network complexity by both the number of hidden layers and the total number of neurons in the network, and measure the GPIA performance against the target model of various complexity. We vary the number of hidden layers from 2 to 8, with 64 neurons at each layer, and use the embedding at the final hidden layer to launch the attack $A_1$. We only consider $A_1$ and $A_2$ in this set of experiments. 

Figure \ref{fig:more-layers} shows the results on Pokec dataset. We observe that both $A_1$ and $A_2$ are less effective on complex GNNs than the simple ones. For example, when the number of hidden layers increases to 8, the  accuracy of both $A_1$ and $A_2$ against GAT becomes close to 0.5.  
 %\xiuling{GraphSAGE aggregates a fixed number of neighbor nodes at each layer, so with the increases of number of layer, more node feature of neighbor nodes will be aggregated. I think the performance GraphSAGE will also be converged to 0.5 with more and more layers. }. 
%Thus the amounts of information encoded in the embedding stay stable regardless the number of hidden layers. 
Although this is against our initial hypothesis that more complex models would intrinsically learn more information from the training dataset and hence be more sensitive to GPIA, our observation is indeed consistent with the prior PIA studies when CNNs are the target model \cite{parisot2021property} that it is not necessary that more complex models are more vulnerable to PIA. 
%However, GPIA performance remains relatively stable when GraphSAGE is the target model, regardless of its number of hidden layers. We believe this is because GraphSAGE only aggregates a fixed number of neighbor nodes at each layer during training. 
% {\bf Main Takeaways.} \Wendy{add main observations of which setup should be used.} \xiuling{For attack classifier, RF is recommended for black-box attacks and MLP is recommended for white-box attacks. For aggregation methods, max-pooling is recommended for embedding aggregation, and concatenation is recommended for posterior aggregation. For embedding dimension alignment method for $A_3$ and $A_4$, TSNE projection is recommended. }

==> text/more-paras.tex <==
\begin{table}[t!]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c}
    \hline
     \multirow{2}{*}{\bf Embedding}&\multicolumn{2}{c|}{\bf GCN} & \multicolumn{2}{c|}{\bf GraphSAGE}&\multicolumn{2}{c}{\bf GAT}  \\ \cmidrule{2-7}
     &$P_1$&$P_4$&$P_1$&$P_4$&$P_1$&$P_4$\\ \cmidrule{1-7}
     $Z^1$&0.98&0.88&0.99&0.76&0.85&0.6\\ \cmidrule{1-7}
     $Z^2$&0.99&0.80&0.99&0.79&0.84&0.59\\ \cmidrule{1-7}
     $Z^3$&0.97&0.76&0.97&0.8&0.82&0.58\\ \cmidrule{1-7}
     $Z^1$, $Z^2$ &0.99&0.88&0.99&0.76&0.85&0.58\\ \cmidrule{1-7}
     $Z^1$, $Z^3$ &0.98&0.89&0.99&0.78&0.83&0.61\\\cmidrule{1-7}
     $Z^2$, $Z^3$ &0.99&0.80&0.99&0.79&0.85&0.58\\ \cmidrule{1-7}
     $Z^1$, $Z^2$, $Z^3$ &0.99&0.87&0.99&0.78&0.86&0.57\\ \hline
    \end{tabular}
    \caption{Impact of amounts of node embeddings on GPIA performance (Pokec dataset). All the GNNs have three hidden layers. Max-pooling is used as the embedding aggregation method. \Wendy{will remove.}}
    \label{tab:more-paras}
    \vspace{-0.2in}
\end{table}


==> text/more-response-for-rebuttal.tex <==
Dear reviewers, thank you for the comments.  Below you can find our response to your questions.

1. We do not assume the attacker has "given all of the nodes in the test graph”. Our assumption is that the attacker has no access to the original nodes in the graph. Instead, he only has access to either the embedding or the posterior probability of these nodes, depending on whether he has the white-box or black-box access to the target model. His goal is to infer the graph properties from either the node embedding or probability values. 

2.	First, we want to point out that the attack accuracy of A3/A4 can be higher than 0.6 in a few settings (e.g., 0.71 in Figure 3 (a) and 0.72 in Figure 3 (b)) when different shadow/target graphs are used. 

Second, we assume that the suggested "train-test leakage" meant the train-test accuracy gap. Indeed we have investigated whether the relatively lower A3/A4 attack accuracy for different shadow/target graphs was led by the train-test gap on these graphs. The results of the A3/A4 attack accuracy values shown in Figure 3 and their associated train-test gap can be found at this anonymous link: https://gitfront.io/r/user-8658281/Ye8LDe7jLN85/GPIA-CCS-REBUTTAL-RESULTS/. We observed that there is no direct relationship between the train-test gap and attack accuracy. Low attack accuracy can be associated with the train-test gap that is either small or large, similarly for high attack accuracy. Therefore we did not include these results in the paper. Instead, we identified the difference in graph characteristics of shadow & target graphs as one reason of the lower A3/A4 attack accuracy (Section 6.2). We can add the results of train-test gap and discussions in the revision. 


==> text/non-binary-PIA.tex <==
\subsection{Beyond Binary PIA: Non-binary PIA on GNNs}
\label{sc:non-binary}

\input{text/non-binary-PIA}

We measure the impact of different number of property classes here, we extend $T_1$ task with $[2,4,6,8]$ classes, the property $p$ is to infer the different between portion of $v_\text{gender='Male'}$ and portion of $v_\text{gender='Female'}$ in a graph. $2$ classes mean $p>0$ or $p\leq0$, $4$ classes mean $p \in \{[-1,-0.5)$ or $[-0.5,0)$ or $[0,0.5)$ or $[0.5,1]\}$, $6$ classes mean $p \in \{[-1,-0.66)$ or $[0.66,-0.33)$ or $[-0.33,0)$ or $[0,0.33)$ or $[0.33,0.66)$ or $[0.66,1]\}$, and $8$ classes follow the same pattern. Each class has the same size of nodes, so the random guess attack accuracy will be 0.5, 0.25, 0.167, 0.125 for 2, 4, 6, 8 property classes respectively. The results are shown in Figure \ref{fig:pia_acc_pclasses}. We observe that a larger number of property classes leads to worse attack accuracy. However they are all above the random guess, especially for the $T_1$ task on GCN, the attack accuracy is stable and close to 1.
\begin{figure*}[t!]
    \centering
%   \vspace{0.1in}
\begin{subfigure}[b]{.7\textwidth}
      \centering
    %  \includegraphics[width=\textwidth]{text/figure/gcn-pia.pdf}
    \includegraphics[width=\textwidth]{text/figure/more-classes-legend(1).pdf}\\
    %  \vspace{-0.2in}
    \end{subfigure}
\begin{tabular}{ccc}
    \begin{subfigure}[b]{.3\textwidth}
      \centering
    %  \includegraphics[width=\textwidth]{text/figure/gcn-pia.pdf}
    \includegraphics[width=\textwidth]{text/figure/gcn-more-classes.pdf}
     \vspace{-0.2in}
    \caption{GCN}
    \end{subfigure}
    &
    \begin{subfigure}[b]{.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{text/figure/gs-more-classes.pdf}
    \vspace{-0.2in}
    \caption{GraphSage}
    \end{subfigure}
    &
    \begin{subfigure}[b]{.3\textwidth} 
    \centering
    \includegraphics[width=\textwidth]{text/figure/gat-more-classes.pdf}
    \vspace{-0.2in}
    \caption{GAT}
    \end{subfigure}
\end{tabular}    
    \vspace{-0.05in}
\caption{\label{fig:pia_acc_pclasses} Attack accuracy of non-binary PIA \Wendy{Add 1 subfigure for link-based attack. Don't use 9 lines. Instead, specify 3 different colors for different GNN, and different line types for different attacks } } 
\end{figure*}



==> text/pia-acc.tex <==

\begin{figure*}[t!]
    \centering
%   \vspace{0.1in}
\begin{subfigure}[b]{.8\textwidth}
      \centering
    %  \includegraphics[width=\textwidth]{text/figure/gcn-pia.pdf}
    \includegraphics[width=\textwidth]{text/figure/pia-legend(4)(1).pdf}
     \vspace{-0.2in}
    \end{subfigure}\\
\begin{tabular}{ccc}
    \begin{subfigure}[b]{.32\textwidth}
      \centering
    %  \includegraphics[width=\textwidth]{text/figure/gcn-pia.pdf}
    \includegraphics[width=\textwidth]{text/figure/gcn-pia2.pdf}
     \vspace{-0.2in}
    \caption{GCN}
    \end{subfigure}
    &
    \begin{subfigure}[b]{.32\textwidth}
    \centering
    % \includegraphics[width=\textwidth]{text/figure/graphsage-pia.pdf}
    \includegraphics[width=\textwidth]{text/figure/gs-pia2.pdf}
    \vspace{-0.2in}
    \caption{GraphSAGE}
    \end{subfigure}
    &
    \begin{subfigure}[b]{.32\textwidth} 
    \centering
    \includegraphics[width=\textwidth]{text/figure/gat-pia2.pdf}
    \vspace{-0.2in}
    \caption{GAT}
    \end{subfigure}
\end{tabular}    
    \vspace{-0.05in}
\caption{\label{fig:pia_acc} Attack accuracy of $A_1$ and $A_2$. $A_1^1$ and $A_1^2$ indicate the attack $A_1$ that uses the model parameters at the 1st and 2nd layer of GNN. $A_1$ and $A_2$ are indicated in different colors respectively, while our approaches, Baseline-1, Baseline-2, and Baseline-3 are indicated in solid fill, horizontal stripe fill, sphere fill, and diagonal shape fill respectively. }
\end{figure*}

\begin{figure*}[t!]
    \centering
%   \vspace{0.1in}
\begin{subfigure}[b]{\textwidth}
      \centering
    %  \includegraphics[width=\textwidth]{text/figure/gcn-pia.pdf}
    \includegraphics[width=\textwidth]{text/figure/pia-acc-more-baseline-legend1.pdf}
     \vspace{-0.2in}
    \end{subfigure}\\
\begin{tabular}{ccc}
    \begin{subfigure}[b]{.32\textwidth}
      \centering
    %  \includegraphics[width=\textwidth]{text/figure/gcn-pia.pdf}
    \includegraphics[width=\textwidth]{text/figure/gcn-4baseline.pdf}
     \vspace{-0.2in}
    \caption{GCN}
    \end{subfigure}
    &
    \begin{subfigure}[b]{.32\textwidth}
    \centering
    % \includegraphics[width=\textwidth]{text/figure/graphsage-pia.pdf}
    \includegraphics[width=\textwidth]{text/figure/gs-acc-more-baseline.pdf}
    \vspace{-0.2in}
    \caption{GraphSAGE}
    \end{subfigure}
    &
    \begin{subfigure}[b]{.32\textwidth} 
    \centering
    \includegraphics[width=\textwidth]{text/figure/gat-acc-more-baseline.pdf}
    \vspace{-0.2in}
    \caption{GAT}
    \end{subfigure}
\end{tabular}    
    \vspace{-0.05in}
\caption{\label{fig:pia_acc_more} Attack accuracy of $A_1$ and $A_2$. $A_1^1$ and $A_1^2$ indicate the attack $A_1$ that uses the model parameters at the 1st and 2nd layer of GNN. $A_1$ and $A_2$ are indicated in different colors respectively, while our approaches, Baseline-1, Baseline-2, Baseline-3, Baseline-4, Baseline-5 are indicated in solid fill, horizontal stripe fill, sphere fill, diagonal shape fill, vertical fill and grid Fill respectively. }
\end{figure*}


\nop{
\begin{figure*}[t!]
    \centering
%   \vspace{0.1in}
    \begin{subfigure}[b]{.49\textwidth}
      \centering
     \includegraphics[width=\textwidth]{text/figure/acc-gcn.pdf}
     \vspace{-0.2in}
    \caption{GCN-Attack accuracy}
    \end{subfigure}
      \begin{subfigure}[b]{.49\textwidth}
         \centering
    \includegraphics[width=\textwidth]{text/figure/f1-gcn.pdf}
    \vspace{-0.2in}
    \caption{GCN-F1 score}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{text/figure/acc-gs.pdf}
    \vspace{-0.2in}
    \caption{GraphSage-Attack accuracy}
    \end{subfigure}
    \begin{subfigure}[b]{.49\textwidth}
      \centering
     \includegraphics[width=\textwidth]{text/figure/f1-gs.pdf}
     \vspace{-0.2in}
    \caption{GraphSage-F1 score}
    \end{subfigure}
    % \vspace{-0.2in}
    \\
    \begin{subfigure}[b]{.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{text/figure/acc-gat.pdf}
    \vspace{-0.2in}
    \caption{GAT-Attack accuracy}
    \end{subfigure}
    \begin{subfigure}[b]{.49\textwidth}
      \centering
     \includegraphics[width=\textwidth]{text/figure/f1-gat.pdf}
     \vspace{-0.2in}
    \caption{GAT-F1 score}
    \end{subfigure}
    \vspace{-0.05in}
\caption{\label{fig:pia_acc} Attack accuracy and F1 score of seven types of attacks under different PIA tasks. } 
\end{figure*}
}


==> text/post-diff-tsne.tex <==
\begin{figure*}[t!]
\centering
%   \vspace{0.1in}
    \centering
       \begin{subfigure}[b]{.15\textwidth}
      \centering
     \includegraphics[width=\textwidth]{text/figure/gcn-pokec-post-diff.png}
     \vspace{-0.2in}
    \caption{$T_1$}
    \end{subfigure}
     \begin{subfigure}[b]{.15\textwidth}
      \centering
     \includegraphics[width=\textwidth]{text/figure/gcn-fb-post-diff.png}
     \vspace{-0.2in}
    \caption{$T_2$}
    \end{subfigure}
    \begin{subfigure}[b]{.15\textwidth}
      \centering
     \includegraphics[width=\textwidth]{text/figure/gcn-pubmed-post-diff.png}
     \vspace{-0.2in}
    \caption{$T_3$}
    \end{subfigure}
    \begin{subfigure}[b]{.15\textwidth}
      \centering
     \includegraphics[width=\textwidth]{text/figure/gcn-pokec2-post-diff.png}
     \vspace{-0.2in}
    \caption{$T_4$}
    \end{subfigure}
     \begin{subfigure}[b]{.15\textwidth}
      \centering
     \includegraphics[width=\textwidth]{text/figure/gcn-fb2-post-diff.png}
     \vspace{-0.2in}
    \caption{$T_5$}
    \end{subfigure}
    \begin{subfigure}[b]{.15\textwidth}
      \centering
     \includegraphics[width=\textwidth]{text/figure/gcn-pubmed2-post-diff.png}
     \vspace{-0.2in}
    \caption{$T_6$}
    \end{subfigure}
\caption{\label{fig:post-diff-gcn} TSNE visualization of the distributions of average difference  in posterior probability of graphs with or w/o property (GNN model: GCN). Blue dots: graphs with property, red dots: graphs without property.}
% \vspace{-0.2in}
\end{figure*}

==> text/pre-attack-obs.tex <==
\subsection{Why does PIA Work (RQ2)?}


\begin{figure*}[t!]
\centering
%   \vspace{0.1in}
    \centering
       \begin{subfigure}[b]{.15\textwidth}
      \centering
     \includegraphics[width=\textwidth]{text/figure/pcn-embed1-pooling-pokec.png}
     \vspace{-0.2in}
    \caption{$T_1,A_1^1$}
    \end{subfigure}
     \begin{subfigure}[b]{.15\textwidth}
      \centering
     \includegraphics[width=\textwidth]{text/figure/pcn-embed2-pooling-pokec.png}
     \vspace{-0.2in}
    \caption{$T_1,A_1^2$}
    \end{subfigure}
    \begin{subfigure}[b]{.15\textwidth}
      \centering
     \includegraphics[width=\textwidth]{text/figure/pcn-posts-pooling-pokec.png}
     \vspace{-0.2in}
    \caption{$T_1,A_2$}
    \end{subfigure}
    \begin{subfigure}[b]{.15\textwidth}
      \centering
     \includegraphics[width=\textwidth]{text/figure/gcn-embed1-pooling-pokec2.png}
     \vspace{-0.2in}
    \caption{$T_4,A_1^1$}
    \end{subfigure}
     \begin{subfigure}[b]{.15\textwidth}
      \centering
     \includegraphics[width=\textwidth]{text/figure/gcn-embed2-pooling-pokec2.png}
     \vspace{-0.2in}
    \caption{$T_4,A_1^2$}
    \end{subfigure}
    \begin{subfigure}[b]{.15\textwidth}
      \centering
     \includegraphics[width=\textwidth]{text/figure/gcn-posts-pooling-pokec2.png}
     \vspace{-0.2in}
    \caption{$T_4,A_2$}
    \end{subfigure}
\caption{\label{fig:dis_pokec} TSNE visualization of the distributions of different inputs of PIA model on different tasks ($T_1$ and $T_4$ on Pokec dataset, GNN model: GCN). Blue dots: graphs with property, red dots: graphs without property. \Wendy{Change (d) - (f) to $T_5$}}
% \vspace{-0.2in}
\end{figure*}

In this part of experiments, we analyze how the graph property impacts the intermediate and final output of the target model, and thus PIA. 

\noindent{\bf Distribution of posterior probability by the target model with vs w/o property} 

\noindent{\bf Distribution of average  difference in posterior probability by the target model with vs w/o property} 
\xiuling{Figure \ref{fig:post-diff-gcn} illustrates the distribution of average  difference in posterior probability for graphs with or w/o property.}
\input{text/post-diff-tsne}



\noindent{\bf Distribution of graph embedding with vs w/o property} 

Figure \ref{fig:dis_pokec} illustrates the distribution of graph embedding (concatenating node emebddings of $\PartialG_i$ after max-pooling) and posteriors (concatenating posteriors of all the nodes in $\PartialG_i$) over the data with and without the property. 



==> text/rebuttal.tex <==
Thanks for the comments. We seek to address the most significant points with clarifications. 

## Reviewer A

**A1 - Intuition behind defense**  

We observed empirically that, interestingly, the defense has disparate effects towards different groups. In particular, adding noise on individual embeddings can mitigate the disparity in node/link influence scores across different groups, which is the key factor of GPIA’s success. We will include these results and analysis in Revision.

## Reviewer B 

 **B1 - Novelty of attacks**

1. Our attack is fundamentally different from existing work in both attack goal and feature design. The existing work only considers *graph-level* properties, with the attack features constructed from a *single* graph embedding, while we consider *group-level* properties, with the attack features constructed from a set of node embeddings. 
2. We are the first to provide comprehensive analysis for better understanding why GPIA works and how it works differently in various settings. 

**B2 - Leakage as an artifact of model**

We have shown the correlation between property features and labels does not contribute to GPIA's success (Section 6.3). Thus the leakage is not an artifact of the model. 

## Reviewer C

**C1 - Property inference vs. feature inference**

Our attack infers the properties directly without inferring feature values first. We will add the feature inference approach as a baseline in Revision.

**C2 – Train/test split**

1. *Train/test split for A3/A4*:  Training and testing data for A3/A4 are sampled from two different graphs, not split from one single graph. 

2. *Access to partial graph in test set*:  The partial graph has access to test set for A1/A2, but not for A3/A4. 
 
3. *Overlap in train & test data*:  The node overlap ratio between training and testing data for Pokec, Facebook, Pubmed datasets is 0.03, 0.05, 0.04 respectively. There is no link overlap between training and testing graphs. We will add these details in Revision. Given the negligible node overlap ratio, we believe the attack accuracy will not be affected much by ensuring no node overlap in the training and testing data. 

**C3 - Better understanding of the attack** 

We will add loss-based influence measurement and loss+threshold approach as a baseline in Revision. Indeed we have additional results showing the group of larger influence is associated with larger average group loss.  

**C4 - Why does transfer attack work?** 

We have additional results showing the disparity in the influence scores across different groups is consistent in both target and surrogate datasets. This shows that GPIA has learned that GNNs behave differently across different groups from the surrogate graph, and transferred this knowledge to target data successfully.  We will add these results in Revision. 

## Reviewer D

**D1 - Assumption of train and test data**

We allow train and test data sampled from two different graphs which have different distributions (attacks A3/A4). 

**D2 - No access to subgraph from same distribution**

We allow subgraph of different distributions (by A3/A4), and have empirical evaluation results for this case (Figure 3). 

**D3 - 50% attack accuracy of baseline**

Not true. Figure 2 shows that the accuracy of some baselines (e.g., Baseline-1/Baseline-2) can be 0.7. 

**D4 - Attack against sparse graph**

We will add results in Revision.

==> text/related-work.tex <==
\section{Related work}
\label{sc:relatedwork}

% \Wendy{Add Missing related work Leakage of Dataset Properties in Multi-Party Machine Learning by Zhang et al. USENIX Security 2021 Property Inference from Poisoning by Mahloujifar et al. IEEE S&P 2022 Formalizing and Estimating Distribution Inference Risks by Suri and Evans PETS 2022}

\noindent{\bf Privacy attacks against graph neural networks. }
Many studies have explored the privacy vulnerability of  GNNs. Based on  which assets in GNN models are considered as sensitive and the adversary tries to obtain, these privacy attacks can be grouped into two categories: 
(1) {\em privacy attacks on GNN models}: the adversary considers GNN models as sensitive (e.g., as the company assets) and aims to extract information about the model’s structure and parameters; and (2) {\em privacy attacks on training data}: the adversary aims to infer the sensitive information in the training graph.  There has been few studies on privacy attacks on GNN models. Wu et al. \cite{wu2021model} design the {\em model extraction attack} that aims to reconstruct a duplicated GNN model. 
In terms of privacy attacks on training data of GNNs, He et al. \cite{he2020stealing} design the link stealing attacks to infer if some specific links exist in the training graph. %They designed 8 different stealing attacks in terms of different adversarial knowledge (the arbitrary combination of node attributes of target dataset, partial graph of target dataset, and shadow dataset). Their attack is based on the foundation that if there is a link between two nodes, their posteriors obtained from the target model should be closer, so they measure the similarity of the posteriors of two nodes, and used unsupervised or supervised model as the attack model. 
Duddu et al. \cite{duddu2020quantifying} design three privacy attacks against GNNs, namely, the {\em membership inference attack} that infer whether a graph node was in the training data, the {\em graph reconstruction attack} that reconstructs the target graph, and the {\em attribute inference attack} to infer the sensitive node attributes.  
He et al. \cite{he2021nodelevel} propose  node-level membership inference attacks against GNNs. Wu et al. \cite{wu2022linkteller} propose a link-level membership inference attack called LINKTELLER to infer the private edge information under the data partition setting where each data holder has either node features or edge information. Zhang et al. \cite{zhang2021inference} design  three types of inference attacks against GNNs: (1) the {\em property inference attack} that infers the sensitive information such as graph density and number of nodes/edges of the training graph; (2) the {\em subgraph inference attack} that aims to infer whether a given subgraph is contained in the original graph; and (3) the {\em graph reconstruction attack} that reconstructs the structure of the training graph. 

Probably the property inference attack in \cite{zhang2021inference} is most relevant to work. Although it shares the same goal as ours, it differs from our attack fundamentally from the following perspective. First,  \cite{zhang2021inference} considers the properties at graph level (e.g., the number of nodes/edges and graph density), while we consider group properties that are defined over groups of nodes and links in the graph. Second,  \cite{zhang2021inference} considers graph embedding (i.e., the vector representation of the whole graph) in the adversary knowledge, while we consider node embeddings that will be available to the adversary in our white-box setting. These major  differences in the type of properties and adversary knowledge lead to fundamentally different design of PIA models.
Furthermore, besides the empirical results to demonstrate the effectiveness of PIA and its defenses, we provide in-depth investigation of which factor(s) contribute to GPIA's success. 

\noindent{\bf Property inference attacks against ML models.}
Ateniese et al. \cite{ateniese2013hacking} first proposed the concept of the  property inference attack against ML models.  They design a white-box PIA model and demonstrate its effectiveness against SVM and HMM models. %However, their attack does not work well on deep neural networks (DNNs). 
%To address this weakness, Ganju et al. \cite{ganju2018property} proposed PIA against  on fully connected neural networks (FCNN). 
%\Wendy{Add discussion of difference between their approach and ours.}
In the following years, the design of PIA has been extended to fully connected neural networks \cite{ganju2018property}, Convolutional Neural Networks (CNNs) \cite{parisot2021property}, collaborative learning  \cite{melis2019exploiting}, federated learning \cite{wang2019eavesdrop,wang2019beyond}, and GANs \cite{zhou2022property}. 
%: class sniffing, quantity inference, and whole determination. Class sniffing detects whether a training label is present within a training round. Quantity inference determines how many clients have a given training label in their dataset. The whole determination infers the global proportion of a specific label. All of those attacks extract properties related to classification labels, and therefore to the main classification task. In contrast，We focus on properties that are, in theory, unrelated to the task of the target model.
%Wang et al. \cite{wang2019beyond} explored user-level privacy leakage against the federated learning. They assumed a malicious server with access to the individual updates, they used updated parameters as input, then trained a variant of GAN with a multi-task discriminator to discriminate category, reality, and client identity of input samples.
%Pejo et al. \cite{pejo2020thegood} proposed quality inference attack, which aimed to recover the quality of the contributing participants’ datasets. They aggregated model updates in each round, and assigned scores to the contributors based on round-wise improvements of testset accuracies.
%Parisot et al. \cite{parisot2021property} studied white-box PIAs on  with image classification as the learning task. They consider the property such as the balanced gender ditribution of images. 
%They took the weights of the target shadow model as input, and trained a meta-classifier to predict whether the training dataset for target model has property P or not. 
%Recently, Melisa et al. \cite{chase2021property} design a property inference poisoning attack where the adversary can maliciously control part of the training data (poisoning data) to increase the leakage of property in the data.  
To the best of our knowledge, there is only one work \cite{zhang2021inference} on the property inference attack against GNNs; the difference between ours and \cite{zhang2021inference} have been discussed above. 
%They generate auxiliary datasets (positive and negative samples) to train a binary classifier attack model. The last one is graph reconstruction attack, which is to reconstruct an adjacency matrix of a graph based on its graph embedding. They train an encoder to generate graph embedding and train a decoder as the attack model (a MLP). 
 
%Third, \cite{zhang2021inference} only presents the empirical evaluation results of PIA effectiveness, while we provide the in-depth analysis of PIA, including the causes of PIA as well as various factors that impact PIA performance.  
%We also design and evaluate new and effective defense mechanisms against the proposed PIA attacks. We note that the defense mechanism in \cite{zhang2021inference} cannot be used in our setting, \Wendy{Explain why.} 
 
%\Wendy{re-read} designed a poisoning approach to do PIA. In their threat model, the adversary added poisoning points in a way that will cause the behavior of the Bayes-optimal classifier to depend on the average of the target property, namely the poisoning would change the prediction of certain instances when the average of property is below the threshold. But when the average is higher than the threshold, then the poisoning does not change the prediction of those points. Based on this designed property of trained Bayes-optimal classifier, then they used black label-only queries on the trained model to determine the frequency of the chosen property of the target dataset. Zhou et al. \Wendy{citation?} propose PIA against GANs, which aims to infer the macro-level training dataset property, i.e., the proportion of samples used to train a target GAN with respect to a certain attribute. They firstly generate latent codes of target training set in full black-box setting or partial black-box settings, then train a property classify based on these latent codes.

 

==> text/summary-of-changes-for-revision.tex <==
"Summary of changes" file can be found at https://docs.google.com/document/d/1EKh-lBDU-klTfyHMvqLhmwz_yO0Ois-z/edit?usp=sharing&ouid=117374505904795675532&rtpof=true&sd=true


1. Clarify attacker model and its practical implications

* Section 5: Clarify the attacker has no access to the original nodes in the graph. Instead, he only has access to either the embedding or the posterior probability of these nodes, depending on whether he has the white-box or black-box access to the target model. His goal is to infer the graph properties from either the node embedding or probability values. 
* Section 5 \& Section 6.1:  Clarify if $G^A$ in A1 \& A2 can have overlapping nodes between training and testing. Also specify that overlapping nodes/links in training and testing data is the worst case for the attack model. 
* Section 5 \& Section 6.1: Clarify if A3 \& A4 have overlapping nodes.  
* Add new results in Section 5 for non-overlapping case.
* Explain why we have overlapping nodes. Also explain how non-overlapping requirements will change the graph characteristics (e.g., node degree, sparsity, etc.)

Practical implications
- Refer to other PIA papers in the literature as the support.
- Explain why property inference should be considered as privacy violation.

2. Train-test leakage 

This should replace discussion of overfitting in Section 6.3. What kind of knowledge is learned from training data that can be carried over to the testing data? Is it because the data with and without the property will have different model accuracy performance? We should add new experiments that measure either the model accuracy or the loss on training data (with property) and testing data (without property). Also add the results of node embeddings generated from data with and without property.  


3. Predicting features from node embeddings.
* Add performance of Baseline method that predicts features from node embeddings in Section 5.
* Add discussions in Section 6.3.
* AIA and PIA use the partial graph of the same size. 

4. Limitations of the attacks 

(1) Node/link overlap between training and testing data (Section 6.4)

(2) Sparse graph (Section 6.4. Maybe optional)

(3) Groups and property of similar size (Table 7 in Section 6.4)

